Overfitting Can Be Harmless for Basis Pursuit, But Only to a Degree

Recently, there have been significant interests in studying the so-called "double-descent" of the generalization error of linear regression models under the overparameterized and overfitting regime, with the hope that such analysis may provide the first step towards understanding why overparameterized deep neural networks (DNN) still generalize well. However, to date most of these studies focused on the min $\ell_2$-norm solution that overfits the data. In contrast, in this paper we study the overfitting solution that minimizes the $\ell_1$-norm, which is known as Basis Pursuit (BP) in the compressed sensing literature. Under a sparse true linear regression model with $p$ i.i.d. Gaussian features, we show that for a large range of $p$ up to a limit that grows exponentially with the number of samples $n$, with high probability the model error of BP is upper bounded by a value that decreases with $p$. To the best of our knowledge, this is the first analytical result in the literature establishing the double-descent of overfitting BP for finite $n$ and $p$. Further, our results reveal significant differences between the double-descent of BP and min $\ell_2$-norm solutions. Specifically, the double-descent upper-bound of BP is independent of the signal strength, and for high SNR and sparse models the descent-floor of BP can be much lower and wider than that of min $\ell_2$-norm solutions.

==> abstract-0602.tex <==
\begin{abstract}

Recently, there have been significant interests in studying the
	generalization power of linear regression models in the
	overparameterized regime, with the hope that such analysis may
	provide the first step towards understanding why overparameterized
	deep neural networks (DNN) generalize well even when they
	overfit the training data. In particular, studies on the min
	$\ell_2$-norm solutions that overfit the training data have
	suggested that such min $\ell_2$-norm solutions exhibit the
	so-called ``double-descent'' behavior, i.e., the test error
	decreases with the number of features $p$ in the
	overparameterized regime when $p$ is much larger than $n$. However,
	for linear models with \emph{i.i.d.} Gaussian features, for
	large $p$ the model errors of such min $\ell_2$-norm solutions
	approach the ``null risk,'' i.e., the error of a trivial
	estimator that always outputs zero, even when the noise is very
	low. In contrast, in this paper we studied the overfitting
	solution that minimizes the $\ell_1$-norm, which is known as
	Basis Pursuit (BP) in the compressed sensing literature. Under a
	sparse true linear model with \emph{i.i.d.} Gaussian features,
	we show that for a large range of $p$ up to a limit that grows
	exponentially with $n$, with high probability the model error of
	BP is upper bounded by a value that not only decreases with $p$,
	but is also proportional to the noise level. To the best of our
	knowledge, this is the first result in the literature showing
	that, without any explicit regularization in such settings where
	both the number of features and the dimension of data are much
	larger than the number of samples, the test errors of a
	practical-to-compute overfitting solution can both exhibit
	double-descent and approach the order of the noise level
	independently of the null risk.  Our upper bound also reveals a
	descent floor for the model error of BP that is proportional to
	the noise level. Further, this descent floor is independent of
	the number of samples $n$ and the null risk, but increases with
	the sparsity level of the true model.

    % Overfitting means interpolating all training data with excessive
	% number of features, which is usually regarded as a situation
	% that needs to be avoided in the field of machine learning.
	% Modern deep neural networks (DNNs) have so many layers and
	% neurons that they are powerful enough to ``memorize" the
	% training data. It is unexpected that DNNs still works well on
	% new test data. Inspired by this, people are wondering whether
	% overfitting can be harmless for some kind of linear
	% regression. Some recent pieces of work show a phenomenon
	% called ``double descent" for min $\ell_2$-norm solution, where
	% the test error decreases on the number of features when the
	% number of features are larger than the number of training
	% data. However, $\ell_2$-norm solution has severe limitations
	% that its test error will soon approach the test error of a
	% trivial zero estimator that always output zero. To avoid that,
	% regularization methods such as LASSO are helpful. However, to
	% work well, those regularization methods need to know
	% parameters like sparsity or noise level in advance, which
	% might be impractical. In this paper, we study Basis Pursuit
	% (BP) for sparse model which has no explicit regularization and
	% does not require those additional information like sparsity or
	% noise level. In this paper, we show that, with Gaussian
	% features, overfitting is harmless for BP within a large range
	% of the number of features, and test error of BP can decrease
	% to the order of noise level. To the best of our knowledge,
	% this is the first paper proving that overfitting can lower the
	% test error to the level of noise, without explicit
	% regularization.
\end{abstract}


==> abstract_arXiv-0602.tex <==
\begin{abstract}
Recently, there have been significant interests in studying the
generalization power of linear regression models in the overparameterized
regime, with the hope that such analysis may provide the first step towards
understanding why overparameterized deep neural networks generalize well even
when they overfit the training data. Studies on min $\ell_2$-norm solutions
that overfit the training data have suggested that such
solutions exhibit the ``double-descent'' behavior, i.e., the test error decreases
with the number of features $p$ in the overparameterized regime when $p$ is
larger than the number of samples $n$. However, for linear models with \emph{i.i.d.}
Gaussian features, for large $p$ the model errors of such min $\ell_2$-norm
solutions approach the ``null risk,'' i.e., the error of a trivial estimator that
always outputs zero, even when the noise is very low. In contrast, we studied
the overfitting solution of min $\ell_1$-norm, which is known as Basis Pursuit
(BP) in the compressed sensing literature. Under a sparse true linear model
with i.i.d. Gaussian features, we show that for a large range of $p$ up to a
limit that grows exponentially with $n$, with high probability the model error
of BP is upper bounded by a value that decreases with $p$ and is proportional
to the noise level. To the best of our knowledge, this is the first result in
the literature showing that, without any explicit regularization in such settings where both $p$
and the dimension of data are much larger than $n$, the test errors of a
practical-to-compute overfitting solution can exhibit double-descent and
approach the order of the noise level independently of the null risk. Our upper
bound also reveals a descent floor for BP that is
proportional to the noise level. Further, this descent floor is independent of~$n$ and the null risk, but increases with the sparsity level of the true model.
\end{abstract}

==> app-lower_bounds-0601.tex <==
\section{Lower bounds}
\label{app:lower_bounds}

We next discuss how tight the upper bounds in the earlier subsections are. Note that $\|w^I\|_1$ and $M$ play key roles in the upper bound in Corollary \ref{coro.wB2_K}. Below, we first show that the upper bounds for $\|w^I\|_1$ (in Proposition \ref{prop.new_WI}) and for $M$ (in Proposition \ref{prop.M}) are quite tight.

A trivial lower bound on $\|w^I\|_1$ is  $\|w^I\|_1\geq \|\etr\|_2$. To realize that, letting $w^I_{(i)}$ denote the $i$-th element of $w^I$, we have
\begin{align*}
    &\|\etr\|_2=\|\Xtr w^I\|_2=\left\|\sum_{i=1}^p w^I_{(i)}\X_i\right\|_2\\
    &\leq \sum_{i=1}^p |w^I_{(i)}|\cdot\|\X_i\|_2=\|w^I\|_1 \text{ (notice $\|\X_i\|_2=1$)}.
\end{align*}
Even by this trivial lower bound, we immediately know that our upper bound on $\|w^I\|_1$ in Proposition \ref{prop.new_WI} is accurate when $p\rightarrow \infty$. Indeed, we can do more than this trivial lower bound, as shown in Proposition \ref{prop.lower_wI} below.


Following the construction of Problem \eqref{prob.temp1}, it is not hard to show that $\mathbf{B}_{(1)}$, i.e., the vector that has the largest inner-product with $(-\etr)$, defines a lower bound for $\|w^I\|_1$.
\begin{lemma}\label{le.true_lower_bound_WI}
\begin{align*}
    \|w^I\|_1\geq \frac{\|\etr\|_2^2}{\mathbf{B}_{(1)}^T(-\etr)}
\end{align*}
\end{lemma}
\begin{proof}
Let
\begin{align*}
    \lambda_*=\frac{(-\etr)}{\mathbf{B}_{(1)}^T(-\etr)}.
\end{align*}
By the definition of $\mathbf{B}_{(1)}$, for any $i\in\{1,2,\cdots, p-s\}$, we have
\begin{align*}
    \left|\lambda_*^T\mathbf{A}_i\right|=\frac{\left|\mathbf{A}_i^T\etr\right|}{|\mathbf{B}_{(1)}^T\etr|}\leq 1.
\end{align*}
In other words, $\lambda_*$ satisfies all constraints of the problem (\ref{prob.dual}), which implies that the optimal objective value of \eqref{prob.dual} is at least
\begin{align*}
    \lambda_*^T(-\etr)=\frac{\|\etr\|_2^2}{\mathbf{B}_{(1)}^T(-\etr)}.
\end{align*}
The result of this lemma thus follows.
\end{proof}

By bounding $\mathbf{B}_{(1)}^T(-\etr)$, we can show the following result.
\begin{proposition}\label{prop.lower_wI}
When $p\leq e^{(n-1)/16}/n$ and $n\geq 17$, then
\begin{align*}
    \frac{\|w^I\|_1}{\|\etr\|_2}\geq \sqrt{1+\frac{n}{9\ln p}}
\end{align*}
with probability at least $1-3/n$.
\end{proposition}
The proof is available in Appendix \ref{app.proof_prop_14}. Comparing Proposition \ref{prop.new_WI} with Proposition \ref{prop.lower_wI}, we can see that, with high probability, the upper and lower bounds of $\|w\|_1$ differ by at most a constant factor.

For $M$, we have the following lemma.
\begin{proposition}\label{le.lower_M}
Assume $p>n$. For any $\delta>0$, there exists a threshold $\tilde{n}$ such that for any $n\geq \tilde{n}$ and $e^{4\delta n}<\lfloor p/2 \rfloor < \exp\left(\frac{2-\sqrt{3}}{4}n\right)$, the following holds.
\begin{align*}
    &\prob{M\geq \frac{\sqrt{2}}{8}\sqrt{\frac{\ln p}{n}}}\geq 1-\exp\left(-\sqrt{p}\right).
\end{align*}
\end{proposition}
Comparing Proposition \ref{prop.M} and with Proposition \ref{le.lower_M}, we can see that when $n$ and $p$ are large, with high probability the upper and lower bounds on $M$ only differ by a constant factor.

The previous discussion suggest that our bounds on $\|w^I\|_1$ and $M$ are quite tight. For Corollary \ref{coro.wB2_K}, however, we do not know how to obtain a matching lower bound on $\|\wBP\|_2$. Still, we conjecture that our lower bound on $\|\wBP\|_2$ may be reasonably tight for the following reasons. First, in Proposition \ref{prop.bound_WB1_KM}, the first term of the upper bound on $\|\wBP\|_1$ is at most a constant multiple of $\|w^I\|_1$ when $K$ is larger than $4$. Intuitive, $w^I$ is a special case of $\wBP$ when the intended signal (i.e., $\beta$) is zero. Thus, we expect that $\|\wBP\|_1$ should be at least on the same order of $\|w^I\|_1$. This suggests that our upper bound on $\|\wBP\|_1$ may be reasonably tight.


\begin{lemma}\label{le.n_plus_s}
There are at most $(n+s)$ non-zero elements in $\wBP$.
\end{lemma}
\begin{proof}
If we prove that
\begin{align}\label{eq.temp_proof_wBP1}
    \wBP_1=\argmin_{w_1}\|w_1\|_1\ \st \Xtr\begin{bmatrix}\wBP_0\\w_1\end{bmatrix}=\etr,
\end{align}
then the result of this lemma follows, since by \eqref{eq.temp_proof_wBP1}, there are at most $n$ non-zero elements in $\wBP_1$.
We now prove \eqref{eq.temp_proof_wBP1} by contradiction. Suppose in contrary that there exist one $w_1^*\neq \wBP_1$ such that
\begin{align*}
    w_1^*=\argmin_{w_1}\|w_1\|_1\ \st \Xtr\begin{bmatrix}\wBP_0\\w_1\end{bmatrix}=\etr.
\end{align*}
Thus, we have
\begin{align*}
    &\|w_1^*\|_1\leq \|\wBP_1\|_1\\
    \implies &\|\wBP_0+\beta_0\|_1+\|w_1^*\|_1\leq \|\wBP_0+\beta_0\|_1+\|\wBP_1\|_1.
\end{align*}
Notice that
\begin{align*}
    \Xtr\begin{bmatrix}\wBP_0\\w_1^*\end{bmatrix}=\etr.
\end{align*}
Therefore, by \eqref{eq.BP_w}, we have
\begin{align*}
    \begin{bmatrix}\wBP_0\\w_1^*\end{bmatrix}=\wBP=\begin{bmatrix}\wBP_0\\\wBP_1\end{bmatrix},
\end{align*}
which implies that $w_1^*=\wBP$, which contradicts our assumption that $w_1^*\neq \wBP_1$.
\end{proof}
By Lemma \ref{le.n_plus_s}, we then have the following lower bound on $\|\wBP\|_2$:
\begin{align}\label{eq.lower_wB2}
    \|\wBP\|_2\geq \frac{\|\wBP\|_1}{\sqrt{n+s}}\geq \frac{\|\wBP\|_1}{\sqrt{2n}}.
\end{align}
By Propositions \ref{prop.wB2_wB1} and \ref{prop.M}, our upper bounds roughly correspond to
\begin{align}\label{eq.temp_0127_2}
    \|\wBP\|_2= \|\etr\|_2+O\left(\sqrt[4]{\frac{\ln p}{n}}\right)\|\wBP\|_1.
\end{align}
Comparing it with \eqref{eq.lower_wB2}, we can see that there is still significant difference between the orders of the factors in front of $\|\wBP\|_1$. Therefore, we cannot rigorously prove that the result in Proposition \ref{prop.wB2_wB1} is tight. However, we conjecture that it is reasonably tight for the following reason. Although there can be $(n+s)$ non-zero elements in $w^{BP}$, we conjecture that the first $s$ elements tend to have more weight than the rest. Therefore, it is likely that
\begin{align}\label{eq.temp_0131_2}
    \|\wBP\|_2\geq \|\wBP_0\|_2\geq \frac{\|\wBP_0\|_1}{\sqrt{s}}=\Omega\left(\frac{1}{\sqrt{s}}\right)\|\wBP\|_1.
\end{align}
By Eq. \eqref{eq.temp_proof_s}, we have
\begin{align*}
    &s\leq \frac{1}{16\sqrt{7}}\sqrt{\frac{n}{\ln p}}\\
    \implies &\frac{1}{\sqrt{s}}=\Omega\left(\sqrt[4]{\frac{\ln p}{n}}\right).
\end{align*}
If Eq. \eqref{eq.temp_0131_2} is true, we will then have
\begin{align*}
    \|\wBP\|_2=\Omega\left(\sqrt[4]{\frac{\ln p}{n}}\right)\|\wBP\|_1,
\end{align*}
which is comparable to Eq. \eqref{eq.temp_0127_2}, and suggests that Proposition \ref{prop.wB2_wB1} may also be reasonably tight. How to rigorously establish Eq. \eqref{eq.temp_0131_2} would be an interesting direction for future work.

% Further, although in general $\|\wBP\|_2$ can be $1/\sqrt{p}$ of $\|\wBP\|_1$, for BP $\wBP$ will mostly concentrate on first $s$ non-sparse elements. Thus, we expect that $\|\wBP\|_2$ should be at least on the order of $\|\wBP\|_1/\sqrt{s}$. This also suggests that our final upper bound on $\|\wBP\|_2$ may be reasonable tight.

{\color{red}
\begin{theorem}[upper bound on $\|\wBP\|_1$]
When $s\leq \sqrt{\frac{n}{7168\ln (16n)}}$, if $p\in \left[(16n)^4,\ \exp\left(\frac{n}{1792s^2}\right)\right]$, then
\begin{align*}
    \|\wBP\|_1\leq \left(4\sqrt{2}+\sqrt{\frac{1}{2\sqrt{7}}}\right)\sqrt{\frac{n}{\ln p}}\|\etr\|_2,
\end{align*}
with probability at least $1-6/p$.
\end{theorem}
\begin{proof}
Following the proof of Theorem~\ref{th.main} in Appendix~\ref{app:proof:main}, we can still get Eq.~(\ref{eq.estimate_M_wI_K}), i.e.,
\begin{align*}
    M\leq 2\sqrt{7}\sqrt{\frac{\ln p}{n}},\ 
    \|w^I\|_1\leq \sqrt{\frac{2n}{\ln p}}\|\etr\|_2,\text{ and }K\geq 4,
\end{align*}
hold with probability at least $1-6/p$.
Applying Eq.~(\ref{eq.estimate_M_wI_K}) in Proposition~\ref{prop.bound_WB1_KM}, with probability at least $1-6/p$, we have
\begin{align*}
    \|\wBP\|_1\leq & 4\|w^I\|_1+\sqrt{\frac{1}{2\sqrt{7}}}\left(\frac{n}{\ln p}\right)^{1/4}\|\etr\|_2\\
    \leq & \left(4\sqrt{2}+\sqrt{\frac{1}{2\sqrt{7}}}\right)\sqrt{\frac{n}{\ln p}}\|\etr\|_2.
\end{align*}
The last inequality is because $\frac{n}{\ln p}>1$, then $(\frac{n}{\ln p})^{1/4}\leq (\frac{n}{\ln p})^{1/2}$.
\end{proof}
\begin{theorem}[lower bound on $\|\wBP\|_1$]\label{th.lower_bound_l1}
When $p\leq e^{(n-1)/16}/n$ and $n\geq 17$, then
\begin{align*}
    \|\wBP\|_1\geq \frac{1}{3}\sqrt{\frac{n}{\ln p}}\|\etr\|_2
\end{align*}
with probability at least $1-3/n$.
\end{theorem}
\begin{proof}
We define
\begin{align*}
    w^J\defeq \argmin_w \|w\|_1\ \st \Xtr w=\etr.
\end{align*}
Because $\Xtr \wBP=\etr$, we have $\|\wBP\|_1\geq \|w^J\|_1$. To get a lower bound on $\|w^J\|_1$, we can directly use\footnote{Notice that in the proof of Proposition~\ref{prop.lower_wI}, we do not require $s>0$. Therefore, we can just let $s=0$ so that $w^I=w^J$.} the result in Proposition~\ref{prop.lower_wI}, i.e.,
\begin{align*}
    \|w^J\|_1\geq \sqrt{1+\frac{n}{9\ln p}}\|\etr\|_2\geq \frac{1}{3}\sqrt{\frac{n}{\ln p}}
\end{align*}
with probability at least $1-3/n$. The result of this proposition thus follows.
\end{proof}
\begin{corollary}[lower bound on $\|\wBP\|_2$]
When $p\leq e^{(n-1)/16}/n$ and $n\geq 17$, then
\begin{align*}
    \|\wBP\|_2\geq \frac{1}{3\sqrt{2}}\sqrt{\frac{1}{\ln p}}\|\etr\|_2
\end{align*}
with probability at least $1-3/n$.
\end{corollary}
\begin{proof}
Applying Eq.~(\ref{eq.lower_wB2}) in Theorem~\ref{th.lower_bound_l1}, we can get the result of this corollary.
\end{proof}
}
\input{simu_wI_M.tex}

==> app_M_lower_bound.tex <==
\section{Proof of Proposition \ref{le.lower_M}}
To prove Proposition \ref{le.lower_M}, we use similar steps and settings as those in Appendix \ref{app.M}. In step 1, we relate the cumulative distribution of $|G_{ij}|$ to the tail probability of $\mathbf{H}_i^T\mathbf{H}_j$. In step 2, we estimate the tail probability of $\mathbf{H}_i^T\mathbf{H}_j$. In step 3, we derive a lower bound on $M$ with high probability. In step 4, we simplify the result derived in step 3. 
\subsection*{Step 1: Relating the cumulative distribution of $|G_{ij}|$ to the tail probability of $\mathbf{H}_i^T\mathbf{H}_j$.}
We have
\begin{align}
    &\prob{|G_{ij}|< a}\nonumber\\
    &=\prob{|G_{ij}|<a,\|\mathbf{H}_i\|_2< \sqrt{2n},\|\mathbf{H}_j\|_2< \sqrt{2n}}\nonumber\\
    &\quad +\prob{|G_{ij}|<a,\{\|\mathbf{H}_i\|_2\geq \sqrt{2n}\text{ or }\|\mathbf{H}_j\|_2\geq\sqrt{2n}\}}\nonumber\\
    &\leq \prob{|\mathbf{H}_i^T\mathbf{H}_j|<2na}+\prob{\|\mathbf{H}_i\|_2>\sqrt{2n}}+\prob{\|\mathbf{H}_j\|_2>\sqrt{2n}}\nonumber\\
    &\qquad \text{ (similar to Eq. \eqref{eq.temp_0129_6} and Eq. \eqref{eq.temp_0129_7} in Appendix \ref{app.M})}\nonumber\\
    &=1-2\prob{\mathbf{H}_i^T\mathbf{H}_j>2na}+2\prob{\|\mathbf{H}_i\|_2>\sqrt{2n}}.\label{eq.temp_0126_4}
\end{align}
Since $\|\mathbf{H}_i\|_2^2$ follows chi-square distribution with $n$ degrees of freedom, we will now use Lemma \ref{le.chi_bound} to bound $\prob{\|\mathbf{H}_i\|_2>\sqrt{2n}}$. Towards this end, notice that
\begin{align}
    &2\sqrt{n\left(\frac{2-\sqrt{3}}{2}n\right)}+2\cdot\frac{2-\sqrt{3}}{2}n\nonumber\\
    =&\left(\sqrt{4-2\sqrt{3}}+2-\sqrt{3}\right)n\nonumber\\
    =&\left(\sqrt{(\sqrt{3}-1)^2}+2-\sqrt{3}\right)n\nonumber\\
    =& n.\label{eq.temp_0126_3}
\end{align}
We then have
\begin{align*}
    &\prob{\|\mathbf{H}_i\|_2\geq\sqrt{2n}}\\
    =&\prob{\|\mathbf{H}_i\|_2^2\geq 2n}\\
    =&\prob{\|\mathbf{H}_i\|_2^2-n\geq 2\sqrt{n\left(\frac{2-\sqrt{3}}{2}n\right)}+2\cdot\frac{2-\sqrt{3}}{2}n}\text{ (by Eq. \eqref{eq.temp_0126_3})}\\
    \leq& \exp\left(-\frac{2-\sqrt{3}}{2}n\right)\text{(by Lemma \ref{le.chi_bound} using $x=\frac{2-\sqrt{3}}{2}n$)}.
\end{align*}
Applying it in Eq. \eqref{eq.temp_0126_4}, we have, for any $i\neq j$,
\begin{align}\label{eq.temp_0126_6}
    \prob{|G_{ij}|< a}\geq 1-2\prob{\mathbf{H}_i^T\mathbf{H}_j>2na}+2\exp\left(-\frac{2-\sqrt{3}}{2}n\right).
\end{align}

\subsection*{Step 2: Estimating the tail probability of $\mathbf{H}_i^T\mathbf{H}_j$.}
We first introduce a lemma as follows, which will be used in estimating the tail probability of $\mathbf{H}_i^T\mathbf{H}_j$.
\begin{lemma}\label{le.temp_0126_le_01}
When $x>0$,
\begin{align*}
    \frac{-1+\sqrt{1+4x^2}}{2x}=\argmax_{\lambda\in (-1,1)}\left(\lambda x-\ln \frac{1}{\sqrt{1-\lambda^2}}\right).
\end{align*}
\end{lemma}
\begin{proof}
Let
\begin{align*}
    f(\lambda)\defeq\lambda x - \ln \frac{1}{\sqrt{1-\lambda^2}}=\lambda x-\frac{1}{2}\ln (1-\lambda^2),\quad \lambda\in(-1,1).
\end{align*}
We have
\begin{align*}
    \frac{df(\lambda)}{d\lambda}&=x-\frac{\lambda}{1-\lambda^2}=\frac{-x\lambda^2-\lambda+x}{1-\lambda^2}.
\end{align*}
Notice that on $\lambda\in(-1, 1)$, the sign of $df/d\lambda$ is the same as that of $g_x(\lambda)\defeq -x\lambda^2-\lambda+x$, which is a quadratic form in $\lambda$. We have $g_x(-1)=1$ and $g_x(1)=-1$.
Therefore, there must exists exactly one $\lambda^*\in(-1, 1)$ such that $g(\lambda^*)=0$, which is given by 
\begin{align*}
    \lambda^*=\frac{-1+\sqrt{1+4x^2}}{2x}\in(-1,1).
\end{align*}
Considering that $g_x(\lambda)$ is the quadratic form of $\lambda$, we have $g_x(\lambda)>0$ for $\lambda\in(-1, \lambda^*)$, and $g_x(\lambda)<0$ for $\lambda\in(\lambda^*, 1)$. Thus, $f(\lambda)$ achieves the maximum at $\lambda^*$.
% Let $df/d\lambda=0$, we have
% \begin{align*}
%     \lambda=\frac{-1\pm \sqrt{1+4x^2}}{2x}.
% \end{align*}
% When $x>0$, we have $f(|\lambda|)\geq f(-|\lambda|)$. Thus, to maximize $f(\lambda)$, we should let
% \begin{align*}
%     \lambda=\frac{-1+\sqrt{1+4x^2}}{2x}.
% \end{align*}
\end{proof}
The following lemma estimates the tail probability of $\mathbf{H}_i^T\mathbf{H}_j$.
\begin{lemma}\label{le.one_column_lower_bound}
Fix $a>0$, for any $\delta>0$, there exists a threshold $\tilde{n}$ such that, for all $n>\tilde{n}$, we have
\begin{align*}
    \prob{\mathbf{H}_i^T\mathbf{H}_j>2na}\geq \exp\left({-n\left(\frac{t-\ln (t/2+1)}{2}+\delta\right)}\right),
\end{align*}
where
\begin{align*}
    t=\sqrt{1+16a^2}-1.
\end{align*}
\end{lemma}
\begin{proof}
Let $Z_k$ be the distribution that corresponds to the product of two random \emph{i.i.d.} standard Gaussian random variables. Then, we know that $\mathbf{H}_i^T\mathbf{H}_j$ are the sum of $n$ independent samples of such $Z_k$'s.
According to Cram\'er's Theorem (Theorem 2.2.3 in \citep{dembolarge}), for any $\delta>0$, there exists a threshold $\tilde{n}$ such that for all $n>\tilde{n}$, we have
\begin{align*}
    \prob{\frac{1}{n}\mathbf{H}_i^T\mathbf{H}_j>2a}\geq e^{-n\left(R+\delta\right)},
\end{align*}
where
\begin{align*}
    R:=&\inf_{x>2a}\sup_{\lambda}\{\lambda x-\ln \mathds{E}[e^{\lambda Z_k}]\}\\
    =&\inf_{x>2a}\sup_{\lambda\in(-1,1)}\left\{\lambda x-\ln \frac{1}{\sqrt{1-\lambda^2}}\right\}\text{ (by Lemma \ref{le.MGF})}.\\
    =&\inf_{x>2a}\frac{1}{2}\left(\sqrt{1+4x^2}-1-\ln \frac{2x^2}{\sqrt{1+4x^2}-1}\right)\text{ (by Lemma \ref{le.temp_0126_le_01})}\\
    =&\inf_{x>2a}\frac{1}{2}\left(\sqrt{1+4x^2}-1-\ln \frac{\sqrt{1+4x^2}+1}{2}\right)\\
    \leq &\frac{1}{2}\left(\sqrt{1+4x^2}-1-\ln \frac{\sqrt{1+4x^2}+1}{2}\right)\bigg|_{x=2a}\text{ (according to the definition of infimum)}\\
    =&\frac{1}{2} (t-\ln (t/2+1)) \text{ (by the choice of $t$ in the lemma)}.
\end{align*}
The conclusion of this lemma thus follows.
\end{proof}

\subsection*{Step 3: Estimating the distribution of $M$.}
We now estimate the distribution of $M$ in the following proposition.
\begin{proposition}\label{prop.temp_0126_1}
For any $\delta>0$, there exists a threshold $\tilde{n}$ such that for any $n\geq \tilde{n}$ and $p\in\{x\mid\frac{\ln\lfloor x/2\rfloor}{n}>2\delta\}$, 
\begin{align}
    &\Pr\left\{\left(M\geq\frac{1}{4} \sqrt{\left(\frac{ \ln\lfloor p/2\rfloor}{n}-2\delta\right)\left(\left(\frac{\ln \lfloor p/2\rfloor}{n}-2\delta\right)+2\right)}\right)\right\}\nonumber\\
    &\geq 1-\exp\left(2\exp\left({-\frac{2-\sqrt{3}}{2}n+\ln \lfloor p/2\rfloor}\right)-2\exp\left(\frac{1}{2}(\ln \lfloor p/2\rfloor)\right)\right).\label{eq.temp_0129_11}
\end{align}
\end{proposition}
\begin{proof}
For any $a>0$ and $\delta>0$, let $\tilde{n}_1$ be the threshold in Lemma \ref{le.one_column_lower_bound}. Then for any $n>\tilde{n}_1$,
we have
\begin{align}
    &\prob{M\geq a}\nonumber\\
    =&1-\Pr\left(\bigcap\limits_{i\neq j}\{|G_{ij}|<a\}\right)\nonumber\\
    \geq &1-\Pr\left(\bigcap\limits_{i\in\{1,\cdots,\lfloor p/2\rfloor\},\ j=i+\lfloor p/2\rfloor}\{|G_{ij}|<a\}\right)\nonumber\\
    = &1-\prob{|G_{1,1+\lfloor p/2\rfloor}|<a}^{\lfloor p/2\rfloor}\text{ (because all $G_{i,i+\lfloor p/2\rfloor}$'s are independent)}\nonumber\\
    \geq & 1- \left(1-2\prob{\mathbf{H}_i^T\mathbf{H}_j>  2na}+2\exp\left(-\frac{2-\sqrt{3}}{2}n\right)\right)^{\lfloor p/2\rfloor}\text{ (by Eq. \eqref{eq.temp_0126_6})}\nonumber\\
    \geq & 1-\left(1+2\exp\left(-\frac{2-\sqrt{3}}{2}n\right)-2\exp\left({-n\left(\frac{1}{2}(t-\ln (t/2+1))+\delta\right)}\right)\right)^{\lfloor p/2\rfloor}\nonumber\\
    &\text{ (by Lemma \ref{le.one_column_lower_bound}, with $t=\sqrt{1+16a^2}-1$ and $n>\tilde{n}_1$)}\nonumber\\
    \geq &1 - \exp\left(\lfloor p/2\rfloor\left[2\exp\left(-\frac{2-\sqrt{3}}{2}n\right)-2\exp\left({-n(\frac{1}{2}(t-\ln (t/2+1))+\delta)}\right)\right] \right)\nonumber\\
    &\text{ (since $1+x\leq e^x$)}\nonumber\\
    = & 1-\exp\left(2\exp\left({-\frac{2-\sqrt{3}}{2}n+\ln \lfloor p/2\rfloor}\right)-2\exp\left[n\left(\frac{\ln \lfloor p/2\rfloor}{n}-\frac{t}{2}+\frac{1}{2}\ln (t/2+1)-\delta\right)\right]\right)\nonumber\\
    \geq & 1-\exp\left(2\exp\left({-\frac{2-\sqrt{3}}{2}n+\ln \lfloor p/2\rfloor}\right)-2\exp\left(n\left(\frac{\ln \lfloor p/2\rfloor}{n}-\frac{t}{2}-\delta\right)\right)\right)\label{eq.temp_0129_10}\\
    &\text{ (since $\ln (t/2+1)\geq 0$)}\nonumber.
\end{align}
Now, we choose
\begin{align}\label{eq.temp_0129_9}
    a=\frac{1}{4}\sqrt{\left(\frac{\ln\lfloor p/2\rfloor}{n}-2\delta\right)\left(\left(\frac{\ln\lfloor p/2\rfloor}{n}-2\delta\right)+2\right)}.
\end{align}
we have
\begin{align*}
    t=&\sqrt{1+16a^2}-1\\
    =&\sqrt{1+\left(\frac{\ln\lfloor p/2\rfloor}{n}-2\delta\right)\left(\left(\frac{\ln\lfloor p/2\rfloor}{n}-2\delta\right)+2\right)}-1\\
    =&\sqrt{\left(\frac{\ln\lfloor p/2\rfloor}{n}-2\delta+1\right)^2}-1\\
    =&\frac{\ln\lfloor p/2\rfloor}{n}-2\delta.
\end{align*}
Thus, we have
\begin{align}\label{eq.temp_0129_8}
    n\left(\frac{\ln \lfloor p/2\rfloor}{n}-\frac{t}{2}-\delta\right)=\frac{\ln \lfloor p/2\rfloor}{2}.
\end{align}
Substituting Eq. \eqref{eq.temp_0129_9} and Eq. \eqref{eq.temp_0129_8} into Eq. \eqref{eq.temp_0129_10}, the result of this proposition thus follows.
\end{proof}

\subsection*{Step 4: Simplifying the expression in Proposition \ref{prop.temp_0126_1}.}
Now we simplify the result in Proposition \ref{prop.temp_0126_1} by using the additional assumption of $e^{4\delta n}<\lfloor p/2 \rfloor < \exp\left(\frac{2-\sqrt{3}}{4}n\right)$ in Proposition \ref{le.lower_M}. We have
\begin{align*}
    -\frac{2-\sqrt{3}}{2}n+\ln \lfloor p/2\rfloor\leq -\frac{2-\sqrt{3}}{4}n.
\end{align*}
Thus, the RHS of Eq. \eqref{eq.temp_0129_11} in Proposition \ref{prop.temp_0126_1} can be relaxed and simplified as follows.
\begin{align*}
    &1-\exp\left(2\exp\left({-\frac{2-\sqrt{3}}{2}n+\ln \lfloor p/2\rfloor}\right)-2\exp\left(\frac{1}{2}(\ln \lfloor p/2\rfloor)\right)\right)\\
    \geq &1-\exp\left(2\exp\left({-\frac{2-\sqrt{3}}{4}n}\right)-2\exp\left(\frac{1}{2}(\ln \lfloor p/2\rfloor)\right)\right)\\
    \geq &1-\exp\left(2\exp\left({-\frac{2-\sqrt{3}}{4}n}\right)-2\exp\left(\frac{1}{2}(\ln\frac{p-1}{2})\right)\right)\\
    &\text{ ($\lfloor p/2\rfloor\geq (p-s)/2$ since $p$ is an integer)}\\
    =& 1-\exp\left(2\exp\left({-\frac{2-\sqrt{3}}{4}n}\right)-\sqrt{2(p-1)}\right).
\end{align*}
As $n$ increases, $\exp\left({-\frac{2-\sqrt{3}}{4}n}\right)$ becomes very small. Also, since $p>n$, by the assumption of the lemma, we can easily find a threshold $\tilde{n}_2$ such that, for all $p>n\geq \tilde{n}_2$, the following holds:
\begin{align*}
    2\exp\left({-\frac{2-\sqrt{3}}{4}n}\right)-\sqrt{2(p-1)}\leq -\sqrt{p}.
\end{align*}
Therefore, the RHS of Eq. \eqref{eq.temp_0129_11} in Proposition \ref{prop.temp_0126_1} can be further relaxed as $1-\exp(-\sqrt{p})$. Now, we simplify the bound of $M$ in Proposition \ref{prop.temp_0126_1}. We have
\begin{align}
    &\frac{1}{4} \sqrt{\left(\frac{ \ln\lfloor p/2\rfloor}{n}-2\delta\right)\left(\left(\frac{\ln \lfloor p/2\rfloor}{n}-2\delta\right)+2\right)}\nonumber\\
    \geq & \frac{1}{4}\sqrt{\frac{\ln \lfloor p/2\rfloor}{2n}\left(\frac{\ln \lfloor p/2\rfloor}{2n}+2\right)}\text{ (because $e^{4\delta n}<\lfloor p/2\rfloor$)}\nonumber\\
    \geq &\frac{1}{4}\sqrt{\frac{\ln \lfloor p/2\rfloor}{n}}\quad\text{ (because $\left(\frac{\ln \lfloor p/2\rfloor}{2n}+2\right)\geq 2$)}.\label{eq.temp_0129_12}
\end{align}
Since $p>n$, we can easily find a threshold $\tilde{n}_3$ such that, for all $p>n\geq \tilde{n}_3$, the following holds:
\begin{align*}
    \ln (p-1)-\ln 2\geq \frac{\ln p}{2},
\end{align*}
which implies that
\begin{align*}
    \frac{\ln p}{2}\leq \ln \frac{p-1}{2}\leq \ln \left\lfloor\frac{p}{2}\right\rfloor.
\end{align*}
Applying it in Eq. \eqref{eq.temp_0129_12}, we have, when $n\geq \tilde{n}_3$,
\begin{align*}
    \frac{1}{4} \sqrt{\left(\frac{ \ln\lfloor p/2\rfloor}{n}-2\delta\right)\left(\left(\frac{\ln \lfloor p/2\rfloor}{n}-2\delta\right)+2\right)}\geq \frac{1}{4}\sqrt{\frac{\ln \lfloor p/2\rfloor}{n}}\geq \frac{\sqrt{2}}{8}\sqrt{\frac{\ln p}{n}}.
\end{align*}
Thus, by choosing $\tilde{n}=\max\{\tilde{n}_1,\tilde{n}_2,\tilde{n}_3\}$, we have, for any $n\geq \tilde{n}$,
\begin{align*}
    &\prob{M\geq \frac{\sqrt{2}}{8}\sqrt{\frac{\ln p}{n}}}\\
    \geq &\prob{M\geq \frac{1}{4} \sqrt{\left(\frac{ \ln\lfloor p/2\rfloor}{n}-2\delta\right)\left(\left(\frac{\ln \lfloor p/2\rfloor}{n}-2\delta\right)+2\right)}}\\
    \geq& 1-\exp\left(-\sqrt{p}\right).
\end{align*}
The conclusion of Proposition \ref{le.lower_M} thus follows.
% \begin{corollary}
% For any $\delta>0$, there exists a threshold $\tilde{n}$ such that for any $n\geq \tilde{n}$ and $e^{4\delta n}<\lfloor p/2 \rfloor < \exp\left(\frac{2-\sqrt{3}}{4}n\right)$, we have
% \begin{align*}
%     &\prob{M\geq \frac{\sqrt{5}}{8}\sqrt{\frac{\ln \lfloor p/2 \rfloor}{n}}}\\
%     &\geq 1-\exp\left(2\exp\left({-\frac{2-\sqrt{3}}{4}n}\right)\right.\\
%     &\left.-2\exp\left(\frac{1}{2}(\ln \lfloor p/2\rfloor)\right)\right).
% \end{align*}
% \end{corollary}

==> auxiliary_result-long.tex <==
\section{Main Ideas of the Proof}
In this section, we present the main ideas behind the proof of Theorem \ref{th.main}. We start with the following definition.

Let
\begin{align}\label{eq.def_WI}
    w^I\defeq\argmin_w\|w\|_1\st \Xtr w=\etr,\ w_0=0.
\end{align}
In other words, $w^I$ is the regressor that fits only the noise.
Note that $w^I$ exists if and only if $p-s\geq n$, which is a little bit stricter than $p > n$. The rest of this paper is based on the condition that $w^I$ exists, i.e., $p-s\geq n$. Notice that in Theorem \ref{th.main}, the condition $p\geq (16n)^4$ already implies that $p\geq (16n)^4\geq 2n\geq s+n$.

The first step (Proposition \ref{prop.bound_WB1_KM} below) is to relate the magnitude of $\wBP$ with the magnitude of $w^I$. The reason that we are interested in this relationship is all follows. Note that one potential way for an overfitting solution to have a small model error is that the solution uses the $p-s$ ``redundant" elements of the regressor to fit the noise, without distorting the $s$ ``significant" elements (that correspond to the non-zero basis of the true regressor). In that case, as $p-s$ increases, it will be easier and easier for the ``redundant" elements of the regressor to fit the noise, and thus the model error may improve with respect to $p$. However, it is not always true that as the ``redundant" elements of the regressor better fit the noise, they do not distort the ``significant" elements of the regressor. Indeed, $\ell_2$-minimization would be such a counter-example: as $p$ increases, although it is easier and easier for the regressor to fit noise, the ``significant" elements of the regressor also go to zero. This is precisely the reason what the min $\ell_2$-norm overfitting solution produces test errors approaching the null risk. In contrast, Proposition \ref{prop.bound_WB1_KM} below shows that this type of undesirable distortion will not occur for BP under suitable conditions. Specifically, define
\begin{align}\label{eq.def_M}
    &M\defeq \max_{i\neq j}\left|\X_i^T\X_j\right|,
\end{align}
where $\X_i$ and $\X_j$ denote $i$-th and $j$-th column of $\Xtr$. Thus, $M$ represents the largest absolute value of inner-product between any two columns of $\Xtr$ (recall that the $\ell_2$-norm of each column is exactly $1$).

Further, let
\begin{align}\label{eq.def_K}
    K\defeq\frac{1+M}{sM}-4.
\end{align}

% The pathway of the proof of Theorem \ref{th.main} consists of following steps:
% \begin{enumerate}
%     \item given $M$, bound $\|\wBP\|_2$ by $\|\wBP\|_1$ (Proposition \ref{prop.wB2_wB1});
%     \item given $M$ and $s$, bound $\|\wBP\|_1$ by $\|w^I\|_1$ (Proposition \ref{prop.bound_WB1_KM});
%     \item bound $\|w^I\|_1$ with $n$ and $p$ (Proposition \ref{prop.new_WI});
%     \item bound $M$ with $n$ and $p$ (Proposition \ref{prop.M}).
% \end{enumerate}
% Notice that we only shows the upper bound of $\|\wBP\|_2$. We have not found an effective lower bound of $\|\wBP\|_2$ or $\|\wBP\|_1$ yet. Thus, whether our bounds on $\|\wBP\|_2$ and $\|\wBP\|_1$ are tight or not is still unclear. In other words, our result in Step 1 and 2 might be improvable. However, we did show that our upper bounds on $\|w^I\|_1$ and $M$ are tight by providing lower bounds on $\|w^I\|_1$ and $M$.

We then have the following proposition that relates the model error $\wBP$ to the magnitude of $w^I$.
\begin{proposition}\label{prop.bound_WB1_KM}
When $K>0$, we must have
\begin{align}\label{eq.prop1}
    \|\wBP\|_1\leq \left(1+\frac{8}{K}+2\sqrt{\frac{1}{K}}\right)\|w^I_1\|_1+\frac{2\|\etr\|_2}{\sqrt{KM}}.
\end{align}
\end{proposition}
Proposition \ref{prop.bound_WB1_KM} shows that, as long as $\|w^I\|_1$ is small, $\|\wBP\|_1$ will also be small. Note that in Eq. \eqref{eq.def_M}, $M$ indicates how similar any two features (that corresponding to the $i$-th and $j$-th columns of $\Xtr$) are. As long as $M$ is much smaller than $1/s$, $M\leq 1/(8s)$ specifically, then the value of $K$ defined in Eq. \eqref{eq.def_K} will be no smaller than $4$. Then, the first term of Eq. \eqref{eq.prop1} will be at most a constant multiple of $\|w^I\|_1$. In conclusion, $\|\wBP\|_1$ will not be much larger than $\|w^I\|_1$ as long as the columns of $\Xtr$ are not very similar.
\begin{proof}
Since we focus on $\wBP$, we rewrite BP in the form of $\wBP$. Notice that
\begin{align*}
    \|\betaBP\|_1=\|\wBP+\beta\|_1=\|\wBP_0+\beta_0\|_1+\|\wBP_1\|_1.
\end{align*}
Thus, we have
\begin{align}\label{eq.BP_w}
    &\wBP=\argmin_w \|w_0+\beta_0\|_1+\|w_1\|_1\nonumber \\
    &\st \Xtr w=\etr.
\end{align}
Define $\mathbf{G}\defeq \Xtr^T\Xtr$ and let $\mathbf{I}$ be the $p\times p$ identity matrix. Let $\abs{\cdot}$ denote the operation that takes component-wise absolute value of every element of a matrix. We have
\begin{align}\label{eq.lemma_begin}
    \|\etr\|_2^2&=\|\Xtr \wBP\|_2^2\nonumber\\
    &=(\wBP)^T\mathbf{G}\wBP\nonumber\\
    &=\|\wBP\|_2^2+(\wBP)^T(\mathbf{G}-\mathbf{I})\wBP\nonumber\\
    &\geq \|\wBP\|_2^2-\abs{\wBP}^T\abs{\mathbf{G}-\mathbf{I}}\abs{\wBP}\nonumber\\
    &\stackrel{(a)}{\geq} \|\wBP\|_2^2-M\abs{\wBP}^T\abs{\mathds{1}-\mathbf{I}}\abs{\wBP}\nonumber\\
    &=(1+M)\|\wBP\|_2^2-M\|\wBP\|_1^2,
\end{align}
where in step (a) $\mathds{1}$ represents a $p\times p$ matrix with all elements equal to $1$, and the step holds because $\mathbf{G}$ has diagonal elements equal to $1$ and off-diagonal elements no greater than $M$ in absolute value.
Because $w^I$ also satisfies the constraint of \eqref{eq.BP_w}, by the representation of $\wBP$ in \eqref{eq.BP_w}, we have
\begin{align*}
    \|\wBP_0+\beta_0\|_1+\|\wBP_1\|_1\leq \|w_0^I+\beta_0\|_1+\|w_1^I\|_1.
\end{align*}
By definition (\ref{eq.def_WI}), we have $w_0^I=\mathbf{0}$ and $\|w_1^I\|_1=\|w^I\|_1$. Thus, we have
\begin{align*}
    \|\wBP_0+\beta_0\|_1+\|\wBP_1\|_1\leq \|\beta_0\|_1+\|w^I\|_1.
\end{align*}
By the triangle inequality, we have $\|\beta_0\|_1-\|\wBP_0+\beta_0\|_1\leq \|\wBP_0\|$. Thus, we have
\begin{align}\label{eq.lemma_second}
    \|\wBP_1\|_1&\leq\|\beta_0\|_1-\|\wBP_0+\beta_0\|_1+\|w^I\|_1\nonumber\\
    &\leq  \|\wBP_0\|_1+\|w^I\|_1.
\end{align}
We now use \eqref{eq.lemma_begin} and \eqref{eq.lemma_second} to establish \eqref{eq.prop1}. Specifically, because $\wBP_0\in \mathds{R}^{s}$, we have
\begin{align*}
    \|\wBP_0\|_2^2\geq \frac{1}{s}\|\wBP_0\|_1^2.
\end{align*}
Thus, we have
\begin{align}\label{eq.temp_1226}
    \|\wBP\|_2^2\geq \|\wBP_0\|_2^2 \geq \frac{1}{s}\|\wBP_0\|_1^2.
\end{align}
Applying Eq. \eqref{eq.lemma_second}, we have
\begin{align}\label{eq.temp_1226_2}
    \|\wBP\|_1=\|\wBP_1\|_1+\|\wBP_0\|_1\leq 2\|\wBP_0\|_1+\|w^I\|_1.
\end{align}
Substituting Eq. \eqref{eq.temp_1226} and Eq. \eqref{eq.temp_1226_2} in Eq. \eqref{eq.lemma_begin}, we have
\begin{align*}
    \frac{1+M}{s}\|\wBP_0\|_1^2-M(2\|\wBP_0\|_1+\|w_1^I\|_1)^2\leq \|\etr\|_2^2,
\end{align*}
which can be rearranged into a quadratic inequality in $\|\wBP_0\|_1$, i.e.,
\begin{align*}
    \left(\frac{1+M}{s}-4M\right)\|\wBP_0\|_1^2&-4M\|w_1^I\|_1\|\wBP_0\|_1\\
    &-\left(M\|w_1^I\|_1^2+\|\etr\|_2^2\right)\leq 0.
\end{align*}
Since $K>0$, we have the leading coefficient $\frac{1+M}{s}-4M>0$. Solving this quadratic inequality for $\|\wBP_0\|_1$ and plugging the result into Eq. \eqref{eq.temp_1226_2}, we have
\begin{align*}
    &\|\wBP\|_1\\
    \leq&\frac{4\|w^I_1\|_1+2\sqrt{4\|w^I_1\|_1^2+K(\|w^I_1\|_1^2+\frac{1}{M}\|\etr\|_2^2)}}{K}+\|w^I\|_1.
\end{align*}
This expression already provides an upper bound on $\|\wBP\|_1$ in terms of $M$ and $\|w^I\|_1$. To obtain an even simpler equation, combing $4\|w^I\|_1/K$ with $\|w^I\|_1$, and breaking apart the square root by $\sqrt{a+b+c}\leq \sqrt{a}+\sqrt{b}+\sqrt{c}$, we have 
\begin{align*}
    % =&\frac{K+4}{K}\|w^I_1\|_1+\sqrt{\left(\frac{4\|w^I\|_1}{K}\right)^2+\frac{4M\|w^I\|_1^2+4\|\etr\|_2^2}{MK}}\\
    \|\wBP\|_1\leq& \frac{K+4}{K}\|w^I\|_1+\sqrt{\left(\frac{4\|w^I\|_1}{K}\right)^2}+\sqrt{\frac{4\|w^I\|_1^2}{K}}\\
    &+\sqrt{\frac{4\|\etr\|_2^2}{MK}}\\
    =&\left(1+\frac{8}{K}+2\sqrt{\frac{1}{K}}\right)\|w^I\|_1+\frac{2\|\etr\|_2}{\sqrt{KM}}.
\end{align*}
\end{proof}

% Normally, we expect that overfitting will be harmless if the ``redundant" elements of the regressor can be used to fit the noise, without affecting the ``significant" elements of the regressor. In that case, as $p$ increases, it will be easier and easier for the ``redundant" elements of the regressor to fit the noise, and thus the test error may improve with respect to $p$. However, it is not always true that as the ``redundant" elements of the regressor better fits the noise, they won't affect the ``significant" elements of the regressor, $\ell_2$-minimization would be such a counter-example: as $p$ increases, although it is easier and easier to fit noise, the ``significant" elements of the regressor also goes to zero. The Proposition \ref{prop.bound_WB1_KM} shows that this undesirable interference will not occur for BP. In other words, as long as $\|w^I\|_1$ is small, $\|\wBP\|_1$ will be small.


Proposition \ref{prop.bound_WB1_KM} only captures the $\ell_1$-norm of $\wBP$. Instead, the test error in Eq. \eqref{eq.testError_w} is directly related to the $\ell_2$-norm of $\wBP$. Proposition \ref{prop.wB2_wB1} below relates $\|\wBP\|_2$ to $\|\wBP\|_1$.

\begin{proposition}\label{prop.wB2_wB1}
\begin{align*}
    \|\wBP\|_2\leq\|\etr\|_2+\sqrt{M}\|\wBP\|_1.
\end{align*}
\end{proposition}
\begin{proof}
In the proof of Proposition \ref{prop.bound_WB1_KM}, we have already proven Eq. \eqref{eq.lemma_begin}. By Eq. \eqref{eq.lemma_begin}, we have
\begin{align*}
    \|\wBP\|_2\leq& \sqrt{\frac{\|\etr\|_2^2+M\|\wBP\|_1^2}{1+M}}\\
    \leq & \sqrt{\|\etr\|_2^2+M\|\wBP\|_1^2}\\
    \leq & \|\etr\|_2+\sqrt{M}\|\wBP\|_1.
\end{align*}
\end{proof}

Note that for an arbitrary vector $\alpha\in\mathds{R}^p$, we can only have $\|\alpha\|_2\leq \|\alpha\|_1$. In contrast, Proposition \ref{prop.wB2_wB1} provides a much tighter bound for $\|\wBP\|_2$ when $M$ is small (i.e., the similarity between the columns of $\Xtr$ is low).





Combining Propositions \ref{prop.bound_WB1_KM} and \ref{prop.wB2_wB1} together, we immediately have the following corollary that relates $\|\wBP\|_2$ to $\|w^I\|_1$.
\begin{corollary}\label{coro.wB2_K}
When $K>0$, we must have
\begin{align*}
    \|\wBP\|_2\leq& \left(1+\frac{2}{\sqrt{K}}\right)\|\etr\|_2\\
    &+\sqrt{M}\left(1+\frac{8}{K}+\frac{2}{\sqrt{K}}\right)\|w^I\|_1.
\end{align*}
\end{corollary}


In order to bound $\|\wBP\|_2$, it only remains to bound $w^I$ and $M$. The following proposition gives an upper bound of $\|w^I\|$.
\begin{proposition}\label{prop.new_WI}
When $n\geq 100$ and $p\geq (16n)^4$, we have
\begin{align}\label{eq.WI}
    \frac{\|w^I\|_1}{\|\etr\|_2}\leq \sqrt{1+\frac{3n/2}{\ln p}},
\end{align}
with probability at least $1-2e^{-n/4}$.
\end{proposition}
% The upper bound in Proposition \ref{prop.new_WI} is decreasing in $p$. It is reasonable because more $p$ means more possible features can be chosen from in order to fit the noise. Since $w^I$ is the solution of minimal $\ell_1$-norm, only $n$ features will be chosen regardless of how large $p$ is. Thus, larger $p$ can only beneficial to get smaller $\|w^I\|_1$. 
Proposition \ref{prop.new_WI} shows that $\|w^I\|_1$ decreases in $p$ at the rate of $O(\sqrt{n/\ln p})$. This is also the reason that $n/\ln p$ shows up in the upper bound in Theorem \ref{th.main}. Further, $\|w^I\|_1$ is proportional to $\|\etr\|_2$, which, when combined with Corollary \ref{coro.wB2_K}, implies that $\|\wBP\|_2$ is on the order of $\|\etr\|_2$. The decrease of $\|w^I\|$ in $p$ is expected by the definition of $w^I$ in \eqref{eq.def_WI} because, when $w^I$ contains more elements, the optimal $w^I$ in \eqref{eq.def_WI} should only have a smaller norm. The contribution of Proposition \ref{prop.new_WI} is in capturing the exact speed with which $\|w^I\|_1$ decreases with $p$, which has not been studied in the literature.
When $p$ approaches $+\infty$, the upper bound in \eqref{eq.WI} becomes $1$. Intuitively, this is because with infinite number of features, eventually there are columns of $\Xtr$ that are very close to $\etr/\|\etr\|_2$. By choosing those columns, $\|w^I\|_1$ approaches $\|\etr\|_2$. 




% \begin{corollary}\label{coro.WI}
% When $n\geq 100$ and $p\in[(16n)^4,\ e^{n/2}]$, then
% \begin{align*}
%     \|w^I\|_1\leq \sqrt{\frac{2n}{\ln p}}\|\etr\|_2,
% \end{align*}
% with probability at least $1-2e^{-n/4}$.
% \end{corollary}
% \begin{proof}
% When $p\leq e^{n/2}$, we have $1\leq \frac{n/2}{\ln p}$. This corollary thus follows.
% \end{proof}

% Proposition \ref{prop.new_WI} gives an upper bound on $\|w^I\|_1$. We also provide an lower bound on $\|w^I\|_1$ in Appendix ??. By comparing the lower and upper bound, we prove that our bounds are precise. 

% Proposition reveals the how well  $\ell_1$-minimization can fit pure noise. Proposition \ref{prop.new_WI} shares some similar features with Theorem \ref{th.main}:
% \begin{enumerate}
%     \item Both bounds on $\wBP$ and $w^I$ are proportional to the noise level $\|\etr\|_2$.
%     \item The term $(n/\ln p)$ appears in both places. Thus, our conjecture about the descent on $p$ and increase on $n$ about $\|\wBP\|_2$ at the end of Section \ref{sec.main_results} also fits here.
% \end{enumerate}
% Those similarities meets our expectation, since solving for $\wBP$ and solving for $w^I$ are kind of doing the same thing: fitting noise while keeping the $\ell_1$ norm of some quantity small. Therefore, as we can prove that the bound on $\|w^I\|_1$ is tight, we have some confidence that our bound on $\|\wBP\|_2$ is precise to some extent.

Finally, the upper bound in \eqref{eq.WI} increases with the number of samples $n$. As we discussed earlier, this is because as $n$ increases, there are more constraints in \eqref{eq.def_WI} for $w^I$ to fit. Thus, the magnitude of $w^I$ increases.

% As we mentioned in the introduction, estimating $w^I$, or equivalently, estimating the least-$\ell_1$ solution of under-determined linear equations, is not an easy job and lacks references. Therefore, the result of estimating $\|w^I\|_1$ is novel and can be viewed as one of our contribution. We will show the methods of estimating $\|w^I\|_1$ in the next section.

The proof of Proposition \ref{prop.new_WI} is also new and quite technical, and will be explained in the next subsection.

Next, we present an upper bound on $M$ as follows.
\begin{proposition}\label{prop.M}
When $p<\exp(n/36)$, we have
\begin{align*}
    \prob{M\leq 2\sqrt{7}\sqrt{\frac{\ln p}{n}}}\geq 1-2e^{-\ln p}-2e^{-n/144}.
\end{align*}
\end{proposition}
It is not hard to verify that for any $i\neq j$, the standard deviation of $\X_i^T\X_j$ equals to $1/\sqrt{n}$.
Since $M$ is defined as the maximum magnitude over $p\times(p-1)$ such pairs of columns, it will grow as some multiple of $1/\sqrt{n}$. Proposition \ref{prop.M} shows that the additional multiplication factor is of the order $\sqrt{\ln p}$.
% Indeed, our estimation on $M$ is also precise in the sense of some constant factor. 
Readers can find detailed proof in Appendix ??.


As $p$ increases, eventually we can find a pair of columns that are closer to each other, which implies that $M$ is large. When some columns of $\Xtr$ are quite similar to the first $s$ columns, BP cannot distinguish the true features. That is the main reason of why the ``double descent" will eventually stop when $p$ is very large, and Theorem \ref{th.main} only hold up to a limit of $p$. 

We are now ready to prove our main result Theorem \ref{th.main}.

\noindent
\begin{myproof}{Theorem \ref{th.main}}
Because 
\begin{align*}
    p\in \left[(16n)^4,\ \exp\left(\frac{n}{1792s^2}\right)\right],
\end{align*}
we have
\begin{align}
    p\geq (16n)^4,\label{eq.temp_proof_p}
\end{align}
and
\begin{align}
    &\exp\left(\frac{n}{1792s^2}\right)\geq p\nonumber\\
    \implies & \frac{n}{1792s^2}\geq \ln p\nonumber\\
    \implies & s\leq \sqrt{\frac{n}{1792\ln p}}=\frac{1}{16\sqrt{7}}\sqrt{\frac{n}{\ln p}}.\label{eq.temp_proof_s}
\end{align}
We also have
\begin{align}
    p\leq \exp\left(\frac{n}{1792s^2}\right)\leq e^{n/1792}.\label{eq.temp_proof_p_u_forM}
\end{align}
Thus, we have
\begin{align}
    &p\leq e^{n/1792}\leq e^{n/2}\nonumber\\
    \implies & 1\leq \frac{n/2}{\ln p}.\label{eq.temp_proof_p_u}
\end{align}

Because $s\leq \sqrt{\frac{n}{7168\ln (16n)}}$, we have
\begin{align}
    n\geq s^2\cdot 7168\ln (16n)\geq 7168>100.\label{eq.temp_proof_n}
\end{align}
Because Eq. \eqref{eq.temp_proof_n} and Eq. \eqref{eq.temp_proof_p}, by Proposition \ref{prop.new_WI}, we have
\begin{align*}
    \|w^I\|_1 &\leq \sqrt{1+\frac{3n/2}{\ln p}}\|\etr\|_2\\
    &\leq \sqrt{\frac{2n}{\ln p}}\|\etr\|_2\text{ (by Eq. \eqref{eq.temp_proof_p_u})}
\end{align*}
with probability at least $1-2e^{-n/4}$, i.e.,
\begin{align}
    \prob{\|w^I\|_1\leq \sqrt{\frac{2n}{\ln p}}\|\etr\|_2}\geq 1-2e^{-n/4}.\label{eq.temp_proof_wI}
\end{align}
Because Eq. \eqref{eq.temp_proof_p_u_forM}, by Proposition \ref{prop.M}, we have
\begin{align}
    \prob{M\leq 2\sqrt{7}\sqrt{\frac{\ln p}{n}}}\geq 1-2e^{-\ln p}-2e^{-n/144}.\label{eq.temp_proof_M}
\end{align}
Notice that for any event $A$ and any event $B$, we have
\begin{align*}
    \proband{A}{B}&=\prob{A}+\prob{B}-\probor{A}{B}\\
    &\geq \prob{A}+\prob{B}-1.
\end{align*}
Thus, by Eq. \eqref{eq.temp_proof_wI} and Eq. \eqref{eq.temp_proof_M} we have
\begin{align*}
    &\proband{\|w^I\|_1\leq \sqrt{\frac{2n}{\ln p}}\|\etr\|_2}{M\leq 2\sqrt{7}\sqrt{\frac{\ln p}{n}}}\\
    &\geq 1-2e^{-n/4}-2e^{-\ln p}-2e^{-n/144}\\
    &\geq 1-6e^{-\ln p}\text{ (by Eq. \eqref{eq.temp_proof_p_u_forM}, $\ln p\leq n/144\leq n/4$)}\\
    &=1-6/p.
\end{align*}
Indeed, if $M\leq 2\sqrt{7}\sqrt{\frac{\ln p}{n}}$,
then we have
\begin{align*}
    K&=\frac{1+M}{sM}-4\text{ (by Eq. (\ref{eq.def_K}))}\\
    &\geq \frac{1}{sM}-4\\
    &\geq \frac{1}{2\sqrt{7}\sqrt{\frac{\ln p}{n}}\cdot \frac{1}{16\sqrt{7}}\sqrt{\frac{n}{\ln p}}}-4\text{ (by Eq. \eqref{eq.temp_proof_s})}\\
    &=8-4=4.
\end{align*}
Therefore, with probability at least $1-6/p$, we have
\begin{align*}
    M\leq 2\sqrt{7}\sqrt{\frac{\ln p}{n}},\ 
    \|w^I\|_1\leq \sqrt{\frac{2n}{\ln p}}\|\etr\|_2,\text{ and }K\geq 4.
\end{align*}
Applying those values in Corollary \ref{coro.wB2_K}, then with probability at least $1-6/p$, we have
\begin{align*}
    \|\wBP\|\leq& 2\|\etr\|_2+\sqrt{2\sqrt{7}}\left(\frac{\ln p}{n}\right)^{1/4}\cdot 4\cdot \sqrt{\frac{2n}{\ln p}}\|\etr\|_2\\
    =& \left(2+8\left(\frac{7n}{\ln p}\right)^{1/4}\right)\|\etr\|_2.
\end{align*}
Dividing both sides by $\|\etr\|_2$, the result of Theorem \ref{th.main} thus follows.

% Then, by Propositions \ref{prop.new_WI} and \ref{prop.M}, we have the following result. If
% \begin{align*}
% (\star)
%     \begin{cases}
%     s\leq \frac{1}{16\sqrt{7}}\sqrt{\frac{n}{\ln p}},\\
%     n>100,\\
%     p\in [(16n)^4,\ e^{n/2}],\\
%     p<\exp(n/36),
%     \end{cases}
% \end{align*}
% then
% \begin{align*}
% (\star\star)
%     \begin{cases}
%     \|w^I\|_1\leq \sqrt{\frac{2n}{\ln p}}\|\etr\|_2 \\
%     \quad \text{ (since $\frac{n/2}{\ln p}\geq 1$ when $p\leq e^{n/2}$)},\\
%     M\leq 2\sqrt{7}\sqrt{\frac{\ln p}{n}},\\
%     K\geq 4,
%     \end{cases}
% \end{align*}
% with the probability at least $(1-2e^{-n/4})(1-2e^{-\ln p}-2e^{-n/144})$. 
% Combining those constraints $(\star)$ together, we know if $p$ exists and
% \begin{align*}
%     p\in \left[(16n)^4,\ \exp\left(\frac{n}{1792s}\right)\right],
% \end{align*}
% then $(\star)$ holds.
% The probability can be estimated as
% \begin{align*}
%     &(1-2e^{-n/4})(1-2e^{-\ln p}-2e^{-n/144})\\
%     \geq & 1-2e^{-\ln p}-4e^{-n/144}\\
%     =& 1- 2/p-4e^{-n/144}\\
%     \geq &1-6/p.
% \end{align*}
% Applying $(\star\star)$ in Corollary \ref{coro.wB2_K}, the result of this theorem thus follows.
\end{myproof}






% \begin{theorem}
% Let
% \begin{align*}
%     C\defeq\frac{1}{5}\left(1-\frac{1}{\sqrt{e}}\right)\sqrt{\frac{2}{\pi}}\approx0.063.
% \end{align*}
% Let
% \begin{align*}
%     M_*\defeq2\sqrt{7}\sqrt{\frac{\ln p}{n}}.
% \end{align*}
% Let
% \begin{align*}
%     K_*\defeq\frac{1+M_*}{sM_*}-4.
% \end{align*}
% When $K^*>0$, and $p-s\geq ne^{9/8}/C$, then
% \begin{align}\label{eq.main_result_1}
%     &\frac{\|\wBP\|_2}{\|\etr\|_2}\leq 1+\frac{2}{\sqrt{K_*}}+\left(1+\frac{8}{K_*}+2\sqrt{\frac{1}{K_*}}\right)\\
%     &\cdot\sqrt{M_*\left(1+\frac{n+\sqrt{2}\sqrt{n-1}}{\left(\sqrt{2\ln\frac{C(p-s)}{n}}-1\right)^2}\right)},
% \end{align}
% with the probability at least
% \begin{align}\label{eq.prob}
%     1-2e^{-n/4}-2e^{-\ln p}-2e^{-n/144}.
% \end{align}
% \end{theorem}

% \begin{corollary}
% Define
% \begin{align*}
%     c\defeq \frac{1}{s}\sqrt{\frac{n}{\ln p}}.
% \end{align*}
% Let $n$ is large. Let
% \begin{align*}
%     1\ll c \leq \frac{1}{s}\sqrt{\frac{n}{2\ln n}}.
% \end{align*}
% (That requires $n^2\leq p\ll \exp\left(\frac{n}{s^2}\right)$.) Then, 
% \begin{align*}
%     \text{RHS of Eq. (\ref{eq.main_result_1})}\approx \sqrt{\frac{c}{\sqrt{2}}}\sqrt{s},\  \text{RHS of Eq. (\ref{eq.prob})}\approx 1.
% \end{align*}
% \end{corollary}
% \begin{proof}
% We have $M_*\approx\sqrt{2}/(cs)$, and $K_*\approx c/\sqrt{2}$. \TODO
% \end{proof}

==> conclusions_copy.tex <==
\section{Conclusions and Future Work}
In this paper, we studied the generalization power of basis pursuit (BP) in the overparameterized regime when the model overfits the data. Under a sparse linear model with \emph{i.i.d.} Gaussian features, we show that the model error of BP not only exhibits ``double descent," but also approaches a descent floor that is on the order of the noise level and independent of the null risk. Further, our analysis reveals important insights on how the descent floor depends on the number of samples, the number of features, and the sparsity level of the true model.

There are several interesting directions for future work. First, it wold be useful to make the discussion in the latter part of Appendix \ref{app:lower_bounds} rigorous, so that we can obtain matching lower bounds on the model error of BP.
Second, we only study the \emph{i.i.d.} Gaussian features in this paper.
It would be important to see if our main conclusions can also be
generalized to other feature models (e.g., Fourier features
\citep{rahimi2008random}), models with mis-specified features
\citep{belkin2019two, hastie2019surprises}, or even the 2-layer neural
network models of \citep{mei2018mean}. 
Finally, we hope that the difference between min $\ell_1$-norm solutions and min $\ell_2$-norm solutions reported here could help us understand the generalization power of overparameterized DNNs, or lead to training methods for DNNs with even better performance in such regimes.
% Third, how BP or min $\ell_1$-norm relates to DNNs?
% Although our results do not provide a direct answer for the generalization power of DNN, we believe that they shed important new insights and raised interesting questions. Given the limitation of the min $\ell_2$-norm solution, is it possible that DNN training is picking some sort of small $\ell_1$-norm solution (or something more general) instead? Alternatively, should we re-engineer the training algorithms so that the model is geared to some sort of min $\ell$-norm solution?

\newpage

\section*{Broader Impact}

Understanding the generalization power of heavily over-parameterized
networks is one of the most foundation aspects of deep learning. By
understanding double descent of generalization errors for Basis Pursuit
(BP) even when it overfits the data, our work advances the understanding
of how such superior generalization power can arise for overfitting
solutions.  Such an understanding will contribute to laying a solid
theoretical foundation of deep learning, which in turn may lead to
practical guidelines in applying deep learning in diverse fields such as 
image processing and natural languages processing.

Controlling the L1-norm also plays a fundamental role in optimization with
sparse models, which have found important applications in, e.g.,
compressive sensing and matrix completion. Without thoroughly studying
the overparameterized regime of BP (which minimizes L1-norm while
overfitting solutions), the theory of double descent remains incomplete.

The insights revealed via our proof techniques in Section 4 (i.e., the
relationship between the error of fitting data and the error of fitting
only noise) not only help to analyze the double descent of BP, but may
also be of value to other more general models. 

Potential negative impacts: Our theoretical results in this paper are
the first step towards understanding the double descent of BP, and
should be used with care. In particular, there is still a significant
gap between our upper and lower bounds, and thus, the significance of
our theories lies more in revealing the general trend rather than
precise characterization of double descent.  Further, the Gaussian model
may also be a limiting factor. Therefore, more efforts will be needed to
sharpen the bounds and generalize the results for applications in
practice.



==> introduction-0602.tex <==
\section{Introduction}

One of the mysteries of deep neural networks (DNN) is that they are not
only over-parameterized so that they can fit the training data (even
perturbed with noise) nearly perfectly, but still produce models that
generalize well to new test data \cite{zhang2016understanding,
advani2017high}. This combination of overfitting and good
generalization challenges the classical wisdom in statistical learning
(e.g., the well-known bias-variance tradeoff) 
\cite{bishop2006pattern, hastie2009elements}. 
%
%In classical statistical learning, it is well understood that there is a
%bias-variance trade-off \cite{bishop2006pattern, hastie2009elements}.
%Thus, when the model has too many parameters (i.e., is
%\emph{overparameterized}), it will produce large variance (despite low
%bias). As a result, although the model can be trained to nearly-zero
%training errors (which is said to have \emph{overfit} the training
%data), it tends to produce large test errors. In order to manage this
%bias-variance trade-off, it is then essential to introduce
%regularization to limit the power of the model so that overfitting does
%not occur
%\cite{hoerl1970ridge,donoho2005stable,zhao2006model,yao2007early,
%meinshausen2009lasso, bickel2009simultaneous}. In contrast, modern DNNs
%have such a large number of layers and neurons that they can essentially
%fit arbitrary functions within a large class \cite{liang2016deep}. In
%that sense, they are powerful enough to ``memorize'' the training data.
%Indeed, even if the training data are perturbed with a significant
%amount of noise, DNNs have no problem in fitting such noisy data with
%zero training error \cite{zhang2016understanding}. It then becomes quite
%unexpected why empirically these networks can still produce good results
%on new test data. 
%
%Unfortunately, the performance of DNNs is difficult to analyze due to
%their non-linearity and non-convexity. 
As a first step towards
understanding why overparameterization and overfitting may be
harmless, a line of recent work has focused on linear regression models 
%with the goal to shed some light on 
\cite{belkin2018understand, belkin2019two,
bartlett2019benign,
hastie2019surprises, mei2019generalization,muthukumar2019harmless}. Indeed, such
results have demonstrated an interesting ``double descent'' phenomenon
for linear models. Roughly
speaking, let $n$ be the number of training samples, and $p$ be the
number of parameters of a linear regression model. As $p$ approaches $n$
from below, the test error of the model (that tries to best fit the
training data) first decreases and then increases to infinity, which is
consistent with the well-understood bias-variance trade-off. As $p$
further increases beyond $n$, overfitting starts to occur (i.e., the
training error will always be zero). However, if one chooses the
overfitting solution that minimizes the $\ell_2$ norm, the test error
decreases again as $p$ increases further. 
%
Such observations, although for models very different from DNN, provide
some hint why overparameterized models may still generalize well. 

To date most studies along this direction have focused on the minimum
$\ell_2$-norm overfitting solutions \cite{belkin2019two,
muthukumar2019harmless,hastie2019surprises,mei2019generalization,mitra2019understanding}. One possible motivation is that, at
least for linear regression problems, 
Stochastic Gradient Descent (SGD), which is often used to
train DNNs, is believed to produce the min $\ell_2$-norm overfitting
solutions
\cite{zhang2016understanding}.
%
%for linear
%models \cite{azizan2018stochastic}, seem to provide a hint why an
%overparameterized DNN may generalize well. 
%
However, it is unclear that SGD will still produce the min $\ell_2$-norm
overfitting solutions for more general models, such as DNN. 
Therefore, it is important to understand whether and how double-descent
occurs for other types of overfitting solutions. Further, the min
$\ell_2$-norm solution usually does not promote sparsity. Instead, it
tends to yield small weights spread across nearly all features, which
leads to distinct characteristics of its double-descent curve (see
further comparisons below). The double-descent of other overfitting
solutions will likely have different characteristics. By understanding
these differences, we may be able to discern which one can potentially
better explain the generalization power of DNN. 


\begin{comment}
However, the analyses in these studies also reveal severe limitations of
the min $\ell_2$-norm overfitting solution. That is, at least for
\emph{i.i.d.} Gaussian features \cite{belkin2019two,
muthukumar2019harmless}, for large $p$ the model error of the min
$\ell_2$-norm overfitting solution quickly approaches the so-called ``null
risk''
\cite{hastie2019surprises}, i.e., the error incurred by a model that
has all zero parameters and always predicts zero. Ideally, if the
training data have lower noise, we would expect that the trained model
would be more accurate and produce lower test errors, instead of
approaching a model of zero estimates and producing a ``null
risk'' that is independent of the noise level. Thus, it would be
much more desirable to establish that the test error of the overfitting
solution can be on the order of the noise level and independent of the
null risk.  \cite{mei2019generalization} studies a more general linear
regression
model for 2-layer neural networks with random (nonlinear) features, 
where the number of features $p$, the number of
samples $n$, and the data dimension $d$ can all vary. (In contrast, the
case of \emph{i.i.d.} Gaussian features can be thought of as $p=d$.)
The ``ridgeless regression'' setting in \cite{mei2019generalization}
also corresponds to min $\ell_2$-norm overfitting solutions. 
The authors
provide sharp asymptotes of the model error as functions of $p/d$ and
$n/d$, when $p, d$, and $n$ all approach infinity. These results suggest
that, for certain ratios of $p/d$ and $n/d$, the asymptotic model error
may approach the order of the noise level. However, when both $p$ and
$d$ are much larger than $n$, the model error will still have a bias
term that does not vanish, which is similar to the ``null risk''
discussed earlier. 
%
\cite{muthukumar2019harmless} studies 
variants of the min $\ell_2$-norm solutions and proves that their model
errors can approach the noise level even when the models overfit.
However, these variants of min $\ell_2$-norm solutions either require
knowledge of the true model in advance, or require an explicit
regularization step (which in turns requires knowledge of the sparsity
and noise levels).
\end{comment}

\begin{comment}
Are there other overfitting solutions whose test errors are on the order
of the noise level? The recent work in \cite{muthukumar2019harmless}
shows that, if one knows the underlying true linear model, then the
solution that minimizes the $\ell_2$-distance to the true model indeed
has test errors that not only follow a ``double-descent'' curve, but
also approach the noise level when $p \to \infty$. However, in practice
this solution cannot be used since we do not know the true model to
begin with. \cite{muthukumar2019harmless} then studies a two-step
procedure: one first finds a regularized solution (e.g., using LASSO),
and then searches for a solution that fits the data but is closest in
$\ell_2$-distance to the regularized solution. When the true model is
sparse, the results in \cite{muthukumar2019harmless} show that such a
two-step procedure can also produce test errors that both follow a
``double-descent'' curve and approach the order of the noise level.
However, this procedure still relies on proper regularization in the
first step, which in turns requires knowledge on the sparsity and the
noise levels. Thus, the results cannot be used to explain why DNN can
work well \emph{without any explicit regularization}. 
\end{comment}

%Given the above limitations of the min $\ell_2$-norm overfitting
%solution, 
In this paper, 
%we are interested in alternative forms of
%overfitting solutions that, without requiring any explicit
%regularization, can not only exhibit double-descent, but also produce
%test errors that are on the order of the noise level and are independent
%of the null risk. 
%%Are there overfitting solutions that can produce test errors on the
%%order of the noise level, without any explicit regularization? Different
%%from the above-cited studies, in this paper 
%In particular, 
we focus on the overfitting
solution with the minimum $\ell_1$-norm. This is known as Basis Pursuit
(BP) in the compressed sensing literature \cite{chen2001atomic}. 
%We are
%interested in whether and how overfitting will be beneficial or harmless
%for BP in linear regression models. 
There are several reasons why we are interested in BP with overfitting.
First, like $\ell_2$-minimization, it does not involve any explicit
regularization parameters, and thus can be used even if we do not know
the sparsity level or the
noise level. Second, it is well-known that using $\ell_1$-norm
promotes sparse solutions \cite{donoho2005stable,zhao2006model, meinshausen2009lasso, bickel2009simultaneous}, which is useful in the
overparameterized regime. 
Third, it is known that the $\ell_1$-norm of the model is
closely related to its ``fat-shattering dimension,'' which is also
related to the Vapnik-Chervonenkis (V-C) dimension and the model capacity 
\cite{bartlett1998sample}. Thus, BP seems to have the
appealing flavor of ``Occam's razor'' \cite{blumer1987occam}, i.e., to
use the simplest explanation that matches the training data.
However, until now the double descent of BP has not been well studied. 
%Although it is still unclear whether DNNs have some yet-to-be-understood inside trick to choose the simplest model
%that fits the training data, by first understanding BP we may shed lights on
%whether or not this line of thinking is a plausible direction to
%explore. 
The numerical results in
\cite{muthukumar2019harmless} suggest that, for a wide range of $p$, BP
indeed exhibits double-descent and produces low test-errors.
%that closely track that of the  proposed there. 
However, no analysis is provided
in \cite{muthukumar2019harmless}. In the compressed sensing literature,
test-error bounds for BP were provided for the
overparameterized regime, see, e.g., \cite{donoho2005stable}.
%where $p$ is much larger than $n$, 
However, the notion of BP there is different as it requires that the
model does
\emph{not} overfit the training data. Hence, such results 
%without strictly interpolating the training data
%\cite{donoho2005stable}. Thus, they 
cannot be used to explain the 
``double-descent'' of BP in the overfitting regime. 
%i.e., why the test error of BP \emph{decreases} with $p$ in the
%overparameterized regime.
To the best of our knowledge, the only work that analyzed the
double-descent of overfitting BP is \cite{mitra2019understanding}. However, the authors only
study the setting where both $n$ and $p$ grow to infinity with a fixed
ratio. As we show later, BP exhibits interesting dynamics of
double-descent when $p$ is exponentially larger than $n$, which
unfortunately collapsed into
a single point of $p/n \to \infty$ in \cite{mitra2019understanding}. 
%
%Thus, to our knowledge, the performance analysis of BP in the
%overfitting regime remains an open problem. 
A thorough study of the double-descen to BP for finite $n$ and $p$ is
still missing. 

The main contribution of this paper is thus to provide new analytical
bounds on the model error of BP in the overfitting regime. As in
\cite{belkin2019two}, we
consider a simple linear regression model with $p$ \emph{i.i.d.}
Gaussian features. We assume that the true model is sparse, and the
sparsity level is $s$. BP is used to train the model by exactly fitting
$n$ training samples. For a range of $p$ up to a value that grows
exponentially with
$n$, we show an upper bound on the model error that decreases with $p$,
which confirms the ``double descent'' phenomenon observed for BP in the
numerical results in \cite{muthukumar2019harmless}. 
To the best of our knowledge, this is the first analytical result in the 
literature establishing the double-descent of min $\ell_1$-norm
overfitting solutions for finite $n$ and $p$. 

Our results reveal significant difference in the double-descent of min
$\ell_1$-norm and $\ell_2$-norm solutions. First, our upper bound for
the model error of BP
is independent of the signal strength (i.e., $||\beta||$ in the model in
Eq.~(\ref{eq.data})). In contrast, the double descent of min $\ell_2$-norm
overfitting solutions usually increases with $||\beta||$, suggesting
that some signals are ``spilled'' into the error of the model. 
Second, the double descent of BP is a lot slower (in $\log p$) than that
of min $\ell_2$-norm overfitting solutions (in $p$). On the other
hand, this also means that the double-descent of BP manifests over a
larger range of $p$ and is easier to observe than that of min
$\ell_2$-norm overfitting solutions. Third, with both $\ell_1$-norm and
$\ell_2$-norm minimization, there is a ``descent floor'' where the model
error reaches the lowest level. However, at high signal-to-noise ratio
(SNR) the descent floor of BP is both lower (by a factor proportional to
$\sqrt{\mathrm{SNR}}$) and wider (for a range of $p$ exponential
in $n$) than that of min $\ell_2$-norm solutions. 

\begin{comment}
That is, 
when $p$
is large, the model error of BP approaches a level on the order of the
noise, with a multiplication factor that only depends on $n$ and $p$ but
is independent of the magnitude of the signal (which equals to the null
risk in our model, see Section~\ref{sec.system_model}). In contrast, the model error of the min
$\ell_2$-norm overfitting solution is usually a function of both the
noise level and the null risk in similar settings \cite{belkin2019two,
hastie2019surprises}.

%To the best of our knowledge, this is the first result in the literature
%showing that, without any explicit regularization (which may require
%knowledge of the sparsity level $s$ and the noise level), in such
%setting where the number of features and the dimension of data are both
%much larger than the number of samples, the test errors of a
%practical-to-compute overfitting solution can exhibit double-descent and
%approach the order of the noise level. 

Several new insights (and
potential limitations) for BP are also revealed by 
our analytical bounds. 
First, for fixed $p$, as the number of
samples $n$ increases, our analytical bound for the model error of BP
also increases, suggesting that the requirement to overfit more data hurts
the performance of BP. 
%While this performance degradation is somewhat disappointing, it is
%actually natural because, as there are more samples, there is also more
%noise that an overfitting solution has to fit. Thus, BP has to ``work
%%harder'' to fit the noise, and as a result produces a larger model error.
However, what is interesting (and perhaps fortunate) is that,
%Second (and perhaps fortunately), 
no matter what the value of $n$ is,
there always exists a range of $p$ (again growing exponentially with
$n$) such that our model-error upper-bound descends to a level
independent of $n$. We refer to this as the ``descent floor.'' In this
sense, an increasing level of overparameterization helps in a
non-trivial manner that ``cancels out'' the additional error
introduced by the
requirement to overfit more data.
We note that min $\ell_2$-norm overfitting solutions also exhibit a
descent floor when the noise is smaller than the signal (the latter again equals
to the null risk). However, as we will elaborate further in Section
\ref{sec.main_results} (see Corollary \ref{coro.only_s}), when the noise
is much smaller than the signal, the descent floor of BP tends to be
significantly lower (because it does not depend on the null risk) and
wider (because of the dependency on $\log p$) than that of min
$\ell_2$-norm solutions.  Second, our upper bound
will hold only for a range of $p$ below a limit that grows exponentially
with $n$. When $p$ grows even larger, eventually BP will pick the wrong
feature and the model error will grow again, which is also observed in
our numerical results. In other words, BP can only sustain ``double-descent'' to some degree (which is nonetheless large). Third, even at the right value of $p$, the
descent floor grows as a $\sqrt{s}$-multiple of the noise level. While
it is not surprising that less-sparse models are harder to learn, it is
still somewhat disappointing that more samples (i.e., larger $n$) does
not help to reduce this descent floor. This observation suggests that,
due to overfitting, BP may not have used the larger number of samples
efficiently. 
\end{comment}

%A key step in the proof of our main results is to establish a 
Our analysis also reveals an interesting 
connection
between the model error of BP and the ability for a min $\ell_1$-norm
solution to fit only the noise. Intuitively, as the number of features
increases, it should become increasingly easier to fit the noise, and thus the
minimum $\ell_1$-norm of such a noise-fitting solution should naturally become smaller. The same is also true for min $\ell_2$-norm solutions.
However, what distinguishes BP is that this ease of fitting noise
directly translates into a smaller model error (see
Proposition~\ref{prop.bound_WB1_KM} in Section~\ref{sect:proof}). In
other words, the BP solution fits the noise in the data without
distorting the true basis much. This behavior appears to be unique to
BP. 
%In contrast, the model error of the min $\ell_2$-norm solution may stay
%at the signal level $||\beta||$ even though the $\ell_2$-norm of a
%noise-fitting solution diminishes to zero \cite{muthukumar2019harmless}.
It would thus be interesting to study whether similar relationships
between the generalization power and the ability to fit noise arise for
other models. 
%including DNNs. 

Finally, our results also reveal limitations of
overfitting, i.e., the descent floor of either BP or min $\ell_2$-norm
solutions cannot be as low as regularized (and non-overfitting)
solutions such as LASSO~\cite{tibshirani1996regression}. However, the type of explicit
regularization used in LASSO is usually not used in DNNs. Thus, it
remains an open question how to find practical overfitting solutions
that can achieve even lower generalization errors without explicit
regularization. 


\begin{comment}
Our work is also related to \cite{mei2019generalization}, which studies
the ``double descent'' phenomenon of two-layer neural networks with
random features at the first layer  and linear weights at the second
layer. \cite{mei2019generalization} focuses on ridge regularization,
which penalizes the training error with $\lambda$ times the
$\ell_2$-norm of regressor. The case of $\lambda \to 0$, i.e., ridgeless
regression, is particularly related to our work as it does not involve
explicit regularization and corresponds to the min $\ell_2$-norm
solution. \cite{mei2019generalization} assumes a model where the number
of features $p$, the number of samples $n$ and the dimension of the
feature $d$ all approach infinity, but keeping $\phi_1=p/d$ and
$\phi_2=n/d$ fixed. It then provides asymptotes of the model error as
functions of $\phi_1$ and $\phi_2$, which also exhibit the
double-descent behavior. Our model in this paper is considerably simpler
as we do not allow non-linear activation functions as in two-layer
neural networks, and we fix $p=d$. Further, we assume in mis-specified
feature in our paper.  Nonetheless, our result illustrates the
difference between using $\ell_1$-norm (as in BP) versus using
$\ell_2$-norm (as in ridge regularization or ridgeless regression).
Specifically, consider the setting where $p$ and $d$ are both larger
than $n$, which is similar to the setting studied in our paper. From the
ridgeless regression (i.e., $\lambda \to 0$) result of Theorem 3 in
\cite{mei2019generalization}, since $\phi_2 = n/d \to 0$, we can show
that the corresponding coefficient for the bias term
($\mathscr{B}_{\text{rless}}$) will approach $1$. As a result, the test
error will not approach the noise level. This behavior  is similar to
the ``null risk'' discussed earlier for the min $\ell_2$-norm
overfitting solution \cite{hastie2019surprises}. In contrast, the
results of our paper show that the min $\ell_1$-norm overfitting
solution (i.e., BP) may produce test errors that approach the noise
level. This difference suggests that, when both the dimension of data
and the number features of the model are much larger than the number of
samples, using the min $\ell_1$-norm solution may be a more effective
alternative.
\end{comment}

\begin{comment}
Finally, our focus on the min $\ell_1$-norm solution is also related to
the recent mean-field studies of two-layer neural networks
\cite{mei2018mean}, where the first-layer weights are trained 
and the second layer performs a linear combining of
the first-layer features but with fixed weights. Note that when the second-layer weights are
fixed, one also bounds the $\ell_1$-norm of the linear weights of
all first-layer features. It would thus be of interest to
revisit how controlling the $\ell_1$-norm plays a role in the
generalization power of such models \cite{bartlett1998sample}.
\end{comment}



==> main_result-0531.tex <==
\section{Main Results}\label{sec.main_results}
Our main result is the following upper bound on the model error of BP with overfitting.
\begin{theorem}[upper bound on $\|\wBP\|_2$]\label{th.main}
When $s\leq \sqrt{\frac{n}{7168\ln (16n)}}$, if $p\in \left[(16n)^4,\ \exp\left(\frac{n}{1792s^2}\right)\right]$, then
\begin{align}\label{eq.main_bound}
    \frac{\|\wBP\|_2}{\|\etr\|_2}\leq 2+8\left(\frac{7n}{\ln p}\right)^{1/4},
\end{align}
with probability at least $1-6/p$.
\end{theorem}
% Although Theorem \ref{th.main} and Corollary \ref{coro.only_s} are only upper bounds instead of the real value of $\|\wBP\|_2$, we are confident that those bounds are relatively precise and informative. Those upper bounds reveals some important features of BP as follows:
Note that the assumption that $s\leq \sqrt{\frac{n}{7168\ln (16n)}}$, which states that the true model is sufficiently sparse, implies that the interval $\left[(16n)^4,\ \exp\left(\frac{n}{1792s^2}\right)\right]$ is not empty. The constants in Theorem \ref{th.main} may be further optimized.

The upper limit of $p$ in Theorem \ref{th.main} thus suggests a descent floor for BP. This leads to the following corollary.
\begin{corollary}\label{coro.only_s}
If $1\leq s\leq \sqrt{\frac{n}{7168\ln (16n)}}$, then by setting $p=\left\lfloor\exp\left(\frac{n}{1792s^2}\right)\right\rfloor$, we have
\begin{align}\label{eq.main_bound_s}
    \frac{\|\wBP\|_2}{\|\etr\|_2}\leq 2+32\sqrt{14}\sqrt{s}
\end{align}
with probability at least $1-6/p$.
\end{corollary}
See Appendix \ref{app.proof_s} for the proof.

{\color{blue}
Theorem~\ref{th.main} and Corollary~\ref{coro.only_s} reveal the following important insights:
\begin{enumerate}
\itemsep 0in
    \item \textbf{Descent floor of BP is independent of $\beta$. In contrast, the descent floor of min $\ell_2$-norm solutions increase with $\beta$.} 
    Corollary \ref{coro.only_s} reveals a descent floor for BP, which is given by $O(\sqrt{s}\|\etr\|_2)$. Note that this descent floor is upper bounded by a value proportional to $\sqrt{s}$ and the noise level $\|\etr\|_2$, but is independent of $n$ and the null risk $\|\beta\|_2$.
    Note that results in \citep{belkin2019two,
hastie2019surprises} suggest that min $\ell_2$-norm solutions also
exhibit a descent floor when $\sigma$ is smaller than $\|\beta\|_2$. The
descent floor occurs at $p/n=\frac{\|\beta\|_2}{|\beta\|_2-\sigma}$, and
is at the level $\sqrt{2\|\beta\|_2\sigma-\sigma^2}$. Compared these two
descent floors, we can see that, when $\sigma\ll \|\beta\|_2$, the
descent floor of BP can be orders-of-magnitude lower than that of min
$\ell_2$-norm solutions. Further, the descent floor of BP is independent
of the null risk $\|\beta\|_2$, which is not the case for min
$\ell_2$-norm solutions. 

\begin{figure}
    \centering
%\vspace{-0.1in}
    \includegraphics[width=5in]{figures/compare_BP_minL2_new}
        \caption{Compare BP with min $\ell_2$-norm, where $\|\etr\|_2=0.01$, $ n=500$.}
        \label{fig.compare_BP_minL2}
\end{figure}
    
    In Fig. \ref{fig.compare_BP_minL2}, we compare BP with the
overfitting solution that minimizes the $\ell_2$-norm. We consider both
the sparse ($s=1$) and not sparse ($s=100$) situations, as well as two
different values of $\|\beta\|_2=1$ and $\|\beta\|_2=0.1$. 
%All four curves
We can observe the descent floors of both algorithms. However,  
comparing the curves with the same $s=100$, we can see that the descent
floors (the lowest points of the curves) of min $\ell_2$-norm solutions vary significantly with
$\|\beta\|_2$, while those of BP are insensitive to $\|\beta\|_2$.
Further, comparing the curves with the same $\|\beta\|_2=1$, we can see
that 
%report the model error $\|w\|_2$ as $p$ increase. Note that all four
%curves decreases sharply when $p$ is a little larger than $n$,
%suggesting the ``double decent" phenomenon.  However, consistent with
%our discussions after Corollary \ref{coro.only_s}, 
the descent floors of
BP are significantly lower and wider than that of min $\ell_2$-norm
overfitting solutions (note that $\|\etr\|_2=0.01\ll \|\beta\|_2=1$).
%Indeed, in the case of $s=1$, the model error of BP keeps decreasing
%within the whole range of $p$ in this figure. 
This result thus
demonstrates the performance advantage of using BP in similar regimes.
% However, we also find significant differences between BP (i.e., minimizing $\ell_1$-norm) and the min $\ell_2$-norm solution. For the min $\ell_2$-norm solution, regardless of $s=1$ or $s=100$, the model error approaches $\|\beta\|_2=1$ (i.e., the ``null risk") when $p$ is large. In the case of $s=100$, although the model error of BP also eventually increases with $p$ (after the decrease at the beginning), BP has a much larger region of descent than that of the min $\ell_2$-norm solution. In the case of $s=1$, the model error of BP keeps decreasing withing the range of $p$ in this figure. In both cases, BP has a lower descent floor than the min $\ell_2$-norm solution.
% In summary, we conclude that, when the number of parameters and the dimension of the data are both much larger than the number of samples, BP performs significantly better than min $\ell_2$-norm solutions in achieving lower model error while overfitting the data.
%
Finally, for the two curves for BP with $\|\beta\|_2=1$ but
different sparsity levels $s$, 
%Next, we
%will show how $s$ affects $\|\wBP\|_2$.  In Fig. \ref{fig.change_s}, we
%draw three curves of $\|\wBP\|_2$ for $s=1$, $s=4$, and $s=16$,
%respectively. We set $\|\beta\|_2=1,\ \|\etr\|_2=0.01$ and $n=100$. The
we can see that the descent floors (the lowest points) 
%%of those three curves are
%$[0.0050, 0.0084, 0.0160]$ for $s=1$, $s=4$, $s=16$ respectively. Thus,
%we find that the descent floor 
are nearly proportional to $\sqrt{s}$, which confirms the result in
Corollary~\ref{coro.only_s}.


    \item \textbf{Descent of BP is slow but easy to observe.}
    The right-hand-side of Eq. (\ref{eq.main_bound}) is monotone decreasing with respect to $p$ (up to a value of $p$ that grows exponentially in $n$). This is consistent with the ``double descent" phenomenon for BP observed in recent numerical experiments in \citep{muthukumar2019harmless}.
    The descent of $\|\wBP\|_2$ happens for a relatively large range of $p$, when $n$ is large and $s$ is relatively small. However, the descent speed is logarithmic in $p$, which is slow and again consistent with the empirical results in \citep{muthukumar2019harmless}.
    Notice that although the descent of BP is slow, Theorem~\ref{th.main} suggests that the descent happens in a large range of $p$. That is why the descent of BP should still be very easy to observe.
    
    Besides Theorem~\ref{th.main} and numerical results (e.g., Fig.~\ref{fig.compare_BP_minL2}), To further support the descent of BP is logarithmic on $p$, we have the following result.
    \begin{corollary}[lower bound on $\|\wBP\|_2$]
When $p\leq e^{(n-1)/16}/n$ and $n\geq 17$, then
\begin{align*}
    \|\wBP\|_2\geq \frac{1}{3\sqrt{2}}\sqrt{\frac{1}{\ln p}}\|\etr\|_2
\end{align*}
with probability at least $1-3/n$.
\end{corollary}
From this lower bound on $\|\wBP\|_2$, we can still find the term $\ln p$ in the denominator, which also validate that the descent of BP is logarithmic slow as $p$ increases.

Readers may have found that there is still a gap between the upper bound and lower bound on $\|\wBP\|_2$, which is true. How to get a matching bound on $\|\wBP\|_2$ could be an interesting future direction. Nonetheless, we still manage to get a matching bound on $\|\wBP\|_1$. Roughly speaking, $\|\wBP\|_1=\Theta(\sqrt{\frac{n}{\ln p}}\|\etr\|_2)$. Although $\|\wBP\|_1$ is not directly related the generalization performance (see Eq.~(\ref{eq.testError_w})), $\|\wBP\|_1$ still quantify how much the BP solution deviates from the true regressor. As $\frac{n}{\ln p}$ (to some power) appears in the matching bound of $\|\wBP\|_1$ just like in the upper bound of $\|\wBP\|_2$ in Theorem~\ref{th.main}, we believe that the bound in Theorem~\ref{th.main} is not terribly bad and insights drawn from Theorem~\ref{th.main} are instructive.
    
    
    
    \item \textbf{Large $n$ increases the model error of BP, but large $p$ compensates it in such a way that the descent floor is independent of $p$.}
    For a fixed $p$ inside the descent region, larger $n$ makes the performance of BP worse. While this may be surprising, it is however reasonable. As $n$ increases, the null space corresponding to Eq. (\ref{eq.BP_constraint}) becomes smaller. Therefore, more data means that BP has to ``work harder" to fit the noise in those data, and consequently BP introduces larger model errors.
    On the positive side, while larger $n$ degrades the performance of BP (due to the requirement of fitting more noise in the training data), the larger $p$ (i.e., overparameterization) helps in a non-trivial way that cancels out the additional increase in model error, so that ultimately the descent floor is independent of $n$. On the negative side, while the increase of the descent floor in $\sqrt{s}$ is not surprising (as less-sparse models are harder to learn), the fact that it does not decrease with $n$ (contrary to, e.g., LASSO \citep{zhao2006model,bickel2009simultaneous, meinshausen2009lasso}) also suggests some inefficiency of BP. That is, due to its overfitting requirement, BP cannot achieve even lower model errors compared to other regularized models (such as LASSO) when more training samples are available.
    
    \item \textbf{The descent floor of BP is lower and wider.}
    Finally, since the model error of BP decreases
in $\log p$, we expect that the descent floor of BP to be significantly
wider than that of min $\ell_2$-norm solutions, which will also be
confirmed numerically in Fig. \ref{fig.compare_BP_minL2}.
\end{enumerate}
}

%  Nonetheless, Theorem \ref{th.main} reveals the following important insights:
% \begin{enumerate}
% \itemsep 0in
%     \item The right-hand-side of Eq. (\ref{eq.main_bound}) is monotone decreasing with respect to $p$ (up to a value of $p$ that grows exponentially in $n$). This is consistent with the ``double descent" phenomenon for BP observed in recent numerical experiments in \citep{muthukumar2019harmless}.
    
%     \item According to Eq. (\ref{eq.main_bound}), $\|\wBP\|_2$ is upper-bounded by a value proportional to $\|\etr\|_2$. Under the normalization procedure in Eq. \eqref{eq.normalize_n} of Section \ref{sec.system_model}, we have $\mathds{E}\|\etr\|_2^2=\sigma^2$. Further, when $n$ is large, $\|\etr\|_2$ and $\sigma$ are close (see Appendix \ref{ap.sec.noise}). Thus, our bound on the model error (and consequently the test error in Eq. (\ref{eq.testError_w})) is on the order of the noise level $\sigma^2$. To the best of our knowledge, this is the first result in the literature showing that, without any explicit regularization in such setting where the number of features and the dimension of data are both much larger than the number of samples,
%     a practical-to-compute overfitting solution can produce test errors approaching the order of the noise level independently of the null risk $\|\beta\|_2$.
    
%     \item The descent of $\|\wBP\|_2$ happens for a relatively large range of $p$, when $n$ is large and $s$ is relatively small. However, the descent speed is logarithmic in $p$, which is slow and again consistent with the empirical results in \citep{muthukumar2019harmless}.
    
%     \item For a fixed $p$ inside the descent region, larger $n$ makes the performance of BP worse. While this may be surprising, it is however reasonable. As $n$ increases, the null space corresponding to Eq. (\ref{eq.BP_constraint}) becomes smaller. Therefore, more data means that BP has to ``work harder" to fit the noise in those data, and consequently BP introduces larger model errors.
    
%     \item Since the sparsity level $s$ does not appear in Eq.  \eqref{eq.main_bound}, we conjecture that the descent speed of $\|\wBP\|_2$ is not sensitive to $s$, as long as $s$ still meets the assumption of Theorem \ref{th.main} that $s=O(\sqrt{n/\ln n})$. However, $s$ may affect the limit of the descent region, as we need $p\leq O(\exp(n/s^2))$.
    
%     \item Our bound only holds for $p\in\left[(16n)^4,\ \exp\left(\frac{n}{1792s^2}\right)\right]$, suggesting that for even larger $p$ the descent will eventually stop. This is because, when there are too many spurious features, eventually some of them will look like the true features. BP may then pick those features and incur a large test error.
% \end{enumerate}



% Corollary \ref{coro.only_s} reveals a descent floor for BP, which is given by $(2+32\sqrt{14}\sqrt{s})\|\etr\|_2$. Note that this descent floor is upper bounded by a value proportional to $\sqrt{s}$ and the noise level $\|\etr\|_2$, but is independent of $n$ and the null risk $\|\beta\|_2$. This corollary has the following implications.
% \begin{enumerate}
% \itemsep 0in
%     \item On the positive side, while larger $n$ degrades the performance of BP (due to the requirement of fitting more noise in the training data), the larger $p$ (i.e., overparameterization) helps in a non-trivial way that cancels out the additional increase in model error, so that ultimately the descent floor is independent of $n$.
    
%     \item On the negative side, while the increase of the descent floor in $\sqrt{s}$ is not surprising (as less-sparse models are harder to learn), the fact that it does not decrease with $n$ (contrary to, e.g., LASSO \citep{zhao2006model,bickel2009simultaneous, meinshausen2009lasso}) also suggests some inefficiency of BP. That is, due to its overfitting requirement, BP cannot achieve even lower model errors compared to other regularized models (such as LASSO) when more training samples are available.
    
%     \item Note that results in \citep{belkin2019two,
% hastie2019surprises} suggest that min $\ell_2$-norm solutions also
% exhibit a descent floor when $\sigma$ is smaller than $\|\beta\|_2$. The
% descent floor occurs at $p/n=\frac{\|\beta\|_2}{|\beta\|_2-\sigma}$, and
% is at the level $\sqrt{2\|\beta\|_2\sigma-\sigma^2}$. Compared these two
% descent floors, we can see that, when $\sigma\ll \|\beta\|_2$, the
% descent floor of BP can be orders-of-magnitude lower than that of min
% $\ell_2$-norm solutions. Further, the descent floor of BP is independent
% of the null risk $\|\beta\|_2$, which is not the case for min
% $\ell_2$-norm solutions. Finally, since the model error of BP decreases
% in $\log p$, we expect that the descent floor of BP to be significantly
% wider than that of min $\ell_2$-norm solutions, which will also be
% confirmed in our numerical results.  \end{enumerate}


==> problem_setting-0531.tex <==
\section{Problem Setting}\label{sec.system_model}
Consider a linear model as follows: 
\begin{align}\label{eq.model}
    y=x^T\underline{\beta}+\ea,
\end{align}
where $x\in\mathds{R}^{p}$ is a vector of $p$ features, $y\in\mathds{R}$ denotes the output, $\ea\in \mathds{R}$ denotes the noise, and $\underline{\beta}\in\mathds{R}^p$ denotes the regressor vector. We assume that each element of $x$ follows \emph{i.i.d.} standard Gaussian distribution, and $\ea$ follows independent Gaussian distribution with zero mean and variance $\sigma^2$. Let $s$ denote the sparsity of $\underline{\beta}$, i.e., $\underline{\beta}$ has at most $s$ non-zero elements. Without loss of generality, we assume that all non-zero elements of $\underline{\beta}$ are in the first $s$ elements. For any $p\times 1$ vector $\alpha$ (such as $\underline{\beta}$), we use $\alpha_0$ to denote the $s\times 1$ vector that consists of the first $s$ elements of $\alpha$, and use $\alpha_1$ to denote the $(p-s)\times 1$ vector that consists of the remaining elements of $\alpha$. With this notation, we have $\underline{\beta}=\left[\begin{smallmatrix}\underline{\beta}_0\\ \mathbf{0}\end{smallmatrix}\right]$.

Let $\underline{\beta}$ be the true regressor and let $\hat{\underline{\beta}}$ be an estimate of $\underline{\beta}$ obtained from the training procedure described below. Let $\underline{w}\defeq \hat{\underline{\beta}}-\underline{\beta}$. According to our model setting, the expected test error satisfies
\begin{align}\label{eq.testError_w}
    &\mathds{E}_{x,\ea}\left[\left(x^T\hat{\underline{\beta}}-(x^T\underline{\beta}+\ea)\right)^2\right]
    =\mathds{E}_{x,\ea}\left[(x^T \underline{w}-\ea)^2\right]
    =\|\underline{w}\|_2^2+\sigma^2.
\end{align}
Since $\sigma^2$ is given, in the rest of the paper we will mostly focus
on the model error $\|\underline{w}\|_2$. Note that if $\hat{\underline{\beta}}=0$, the model error equals to $\|\underline{\beta}\|_2$ which is the $\ell_2$-norm of the signal $x^T
\underline{\beta}$, and is referred to as the ``null risk'' \citep{hastie2019surprises}.

We next describe how BP computes $\hat{\underline{\beta}}$ from training data. The training data is given by $(\Xtr$,  $\Ytr)$, where $\Xtr\in\mathds{R}^{n\times p}$ and $\Ytr\in\mathds{R}^n$. For ease of analysis, we normalize each column of $\Xtr$ as follows.

% Each row of $\Xtr$ and $\Ytr$ corresponds to a (scaled) sample of $x^T$ and $y$, respectively. We use a $p\times 1$ vector  $\etr$ to denote the noise in the training data. Then, the training data can also be written as
% \begin{align}\label{eq.data}
%     \Ytr= \Xtr\beta+\etr.
% \end{align}
% Given $\Xtr$ and $\Ytr$, our job is to find an estimator $\hat{\beta}$ for $\beta$ even though we do not know $\etr$. As is common in compressed sensing \citep{donoho2005stable}, we assume that each column of $\Xtr$ is normalized. That is, we 

Assume that we have $n$ \emph{i.i.d.} samples in the form of Eq.~(\ref{eq.model}). For each sample $j$, we first divide both sides of Eq. (\ref{eq.model}) by $\sqrt{n}$, i.e.,
\begin{align}\label{eq.normalize_n}
    \frac{y_j}{\sqrt{n}}=\left(\frac{x_j}{\sqrt{n}}\right)^T\underline{\beta} + \frac{\ea_j}{\sqrt{n}}.
\end{align}


We then form a matrix $\mathbf{H}\in\mathds{R}^{n\times p}$ so that each row $j$ is the sample $x_j^T$. Writing $\mathbf{H}=[\mathbf{H}_1\ \mathbf{H}_2\ \cdots\ \mathbf{H}_p]$,
we then have $\mathds{E}[\|\mathbf{H}_i\|_2^2]=n$, for each column $ i\in\{1,2,\cdots,p\}$. Now, let $\Xtr=[\X_1\ \X_2\ \cdots\ \X_p]$ be constructed in such a way that
\begin{align}\label{def.norm_X}
    \X_i=\frac{\mathbf{H}_i}{\|\mathbf{H}_i\|_2},\ \forall i\in\{1,2,\cdots,p\},
\end{align}
and let each row $j$ of $\Ytr$ and $\etr$ be the corresponding values of $y_j/\sqrt{n}$ and $\ea_j/\sqrt{n}$ of the sample. Then, each column $\X_i$ will have a unit $\ell_2$-norm. We can then write the training data as
\begin{align}\label{eq.data}
    \Ytr= \Xtr\beta+\etr,
\end{align}
where
\begin{align}
    \beta_{i} = \frac{\|\mathbf{H}_i\|_2}{\sqrt{n}}\underline{\beta}_i\ \forall i\in \{1,2,\cdots, p\}.\label{eq.scale_beta}
\end{align}
Note that the above normalization of $\Xtr$ leads to a small distortion from $\underline{\beta}$ to $\beta$, but it eases our subsequent analysis. When $n$ is large, the distribution is small, which will be make precise below (in Lemma xx).

% Note that this normalization procedure distorts the value of $\beta$ in Eq. (\ref{eq.data}) from the original value in Eq. (\ref{eq.model}). However, when $n$ is large, the distortion is small. Since we focus on the model error $\|w\|_2=\|\beta-\hat{\beta}\|_2$, the normalization will not qualitatively affect the main conclusions of the paper. {\color{red}We defer the rigorous proof on this claim in Appendix~\ref{app.normalize}.}



In the rest of this paper, we focus on the situation of overparameterization, i.e., $p>n$. Among many different estimators of $\beta$, we are interested in those that perfectly fit (i.e., overfit) the training data, i.e., 
\begin{align}\label{eq.BP_constraint}
    \Xtr\hat{\beta}=\Ytr.
\end{align}
When $p>n$, there are infinitely many $\hat{\beta}$'s that satisfy Eq. \eqref{eq.BP_constraint}. In BP \citep{chen2001atomic}, $\hat{\beta}$ is chosen by solving the following problem
\begin{align}\label{eq.BP_origin}
    \betaBP \defeq \argmin_{\tilde{\beta}}\|\tilde{\beta}\|_1\ \st \Xtr\tilde{\beta}=\Ytr.
\end{align}
In other words, given $\Xtr$ and $\Ytr$, BP finds the overfitting solution $\betaBP$ with the minimal $\ell_1$-norm.
Define $\wBP\defeq \betaBP-\beta$. In the rest of our paper, we will show how to estimate the model error $\|\wBP\|_2$ of BP as a function of the system parameters such as $n$, $p$, $s$, and $\sigma^2$. 
Note that before we apply the solution of BP in Eq.~(\ref{eq.BP_origin}) to new test data, we should re-scale it back (see Eq.~(\ref{eq.scale_beta})) to
\begin{align*}
    \underline{\betaBP}_{i}=\frac{\sqrt{n}\betaBP_i}{\|\mathbf{H}_i\|_2},\ \forall i\in \{1,2,\cdots, p\}.
\end{align*}
and measure the generalization performance by the unscaled version of $\wBP$, i.e.,  $\underline{\wBP}=\underline{\betaBP}-\underline{\beta}$. The following lemma shows that, when $n$ is large, the difference of $\ell_1$-norm and $\ell_2$-norm between $\wBP$ and $\underline{\wBP}$ is within a factor of $\sqrt{2}$ with high probability.
\begin{lemma}
For both $i=1$ and $i=2$, we have
\begin{align*}
    &\prob{\|\underline{\wBP}\|_i\leq \sqrt{2}\|\wBP\|_i}\geq 1-\exp\left(-\frac{n}{16}+\ln (2n)\right),\\
    &\prob{\|\wBP\|_i\leq \sqrt{2}\|\underline{\wBP}\|_i}\geq 1-\exp\left(-\frac{2-\sqrt{3}}{2}n+\ln (2n)\right).
\end{align*}
\end{lemma}
Therefore, in the rest of the paper we will focus on $\wBP$.


Note that \citep{donoho2005stable} also studies the model error of BP. However, the notion of BP there is different. In particular, the estimator $\hat{\beta}$ only needs to satisfy $\|\Ytr-\Xtr\hat{\beta}\|_2\leq\delta$. The main result there, i.e., Theorem 3.1 of \citep{donoho2005stable}, requires $\delta$ to be greater than the noise level $\|\etr\|_2$ (and thus cannot be zero). Therefore, the result of \citep{donoho2005stable}\footnote{The earlier version of \citep{donoho2005stable} has a mistake on claiming that $\delta$ can be zero for $\epsilon>0$.} does not capture the performance of BP for the overfitting setting stated in Eq. (\ref{eq.BP_constraint}).








==> simu_wI_M.tex <==
\begin{figure}
    \centering
    \begin{minipage}[t]{0.47\textwidth}
        \centering
        \includegraphics[width=2.8in]{figures/w_I.eps}
        \caption{Bounds of $\|w^I\|_1$ and its exact value, where $\|\etr\|_2=0.01$, $ n=20$.}
        \label{fig.wI}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.47\textwidth}
        \centering
        \includegraphics[width=2.8in]{figures/M.eps}
        \caption{The value of $M$ and its upper bounds (given in Proposition \ref{prop.M}) for the cases of $n=300$ and $n=1200$.}
        \label{fig.M}
    \end{minipage}
\end{figure}

\begin{figure}
    \centering
%\vspace{-0.1in}
    \includegraphics[width=3.5in]{figures/wB.eps}
        \caption{Exact values and upper bounds of $\|\wBP\|_2$ for cases of $s=1$ and $s=2$, where  $\|\beta\|_2=1$, $\|\etr\|_2=0.01$, $n=3000$.}
        \label{fig.WB}
\end{figure}

In Fig. \ref{fig.wI}, we draw the lower and upper bounds on $\|w^I\|_1$ as $(p-s)$ increases, for the setting of $\|\etr\|_2=0.01$ and $n=20$. The blue curve ``ub, Prop. \ref{prop.bound_WI1}" denotes our theoretical upper bound on $\|w^I\|_1$ (here we use a more detailed form that is tighter than Proposition \ref{prop.new_WI}, which is given in Proposition \ref{prop.bound_WI1} in Appendix \ref{app.proof_of_lemma_12}). 
In the proof of Proposition \ref{prop.new_WI}, we use the idea that $\|w^I\|_1$ is mostly determined by the columns of $\Xtr$ that are closest to the direction of $\etr$. Specifically, among the last $(p-s)$ columns of $\Xtr$, we order them based on the absolute values of their inner-products with $\etr$, and choose $5n$ columns $\mathbf{B}_{(1)},\cdots,\mathbf{B}_{(5n)}$ with the largest values such that $|\mathbf{B}_{(1)}^T\etr|\geq|\mathbf{B}_{(2)}^T\etr|\geq\cdots\geq|\mathbf{B}_{(5n)}^T\etr|$. The upper bounds in Propositions \ref{prop.bound_WI1} and \ref{prop.new_WI} are derived based on the probability distribution of these columns. In contrast, using the \emph{exact} values of these columns, we can construct even tighter bounds on $\|w^I\|_1$. Specifically, in Fig. \ref{fig.wI}, the yellow curve ``ub, use $\mathbf{B}_{(5n)}$" denotes a tighter upper bound on $\|w^I\|_1$ constructed by using the exact value of $\mathbf{B}_{(5n)}$ (see Corollary \ref{coro.bound_by_Aq} in Appendix \ref{app:proof:wI}). The green curve ``ub, use $\mathbf{B}_{(1)}$ to $\mathbf{B}_{(5n)}$" denotes yet another upper bound on $\|w^I\|_1$ constructed by using the exact values of  $\mathbf{B}_{(1)},\cdots, \mathbf{B}_{(5n)}$ (see problem \eqref{prob.temp1} in Appendix \ref{app:proof:wI}). The red curve ``real value" denotes the real value of $\|w^I\|_1$. The purple curve ``lb, use $\mathbf{B}_{(1)}$" denotes the lower bound in Lemma \ref{le.true_lower_bound_WI} of Appendix \ref{app:lower_bounds} using the exact value of $\mathbf{B}_{(1)}$. The first thing that we can verify is that $\|w^I\|_1$ decreases when $(p-s)$ increases. Further, the speed of decrease is relatively slow (notice that the x-axis is in $\log$ scale). In Fig. \ref{fig.wI}, we can see that all curves gets closer when $p$ increases, which implies that our upper bound on $\|w^I\|_1$ is tight. Further, we find that the upper bound using $\mathbf{B}_{(1)}$ to $\mathbf{B}_{(5n)}$ (green curve) almost overlaps with the exact value of $\|w^I\|_1$ (red curve), which verifies our intuition that these columns determine the value of $\|w^I\|_1$.

In Fig. \ref{fig.M}, we compare the upper bound on $M$ (given in Proposition \ref{prop.M}) with its exact value. We show two cases, $n=300$ (red curves) and $n=1200$ (blue curves). For each case, we can see that the derived upper bound and the exact value of $M$ only differ by a constant factor, which verifies the tightness of our upper bound on $M$ in Proposition \ref{prop.M}.
% When $p=10^4$, those four curves have the value $[1.85, 0.701, 0.496, 0.253]$, from the highest to the lowest, respectively. 
The curve of the exact value of $M$ for $n=1200$ also differs with that for $n=300$ by a constant factor, which is close to $2=\sqrt{1200/300}$. This figure thus validates our conclusion that $M$ is approximately proportional to $1/\sqrt{n}$ for a fixed $p$.

In Fig. \ref{fig.WB}, we draw the value of $\|\wBP\|_2$ and its upper bound in Corollary \ref{coro.wB2_K} for cases of $s=1$ and $s=2$. 
All curves are computed using the exact value of $M$ and $\|w^I\|_1$, since we have already shown that our estimates on $M$ and $\|w^I\|_1$ are tight. We see that there is still a relatively large gap between our bound and the real value of $\|\wBP\|$ suggesting room for more refined analysis. 
% One possible reason is that, $n$ is not big enough, thus $K$ in Corollary \ref{coro.wB2_K} introduce a relatively significant constant factor. In Fig. \ref{fig.WB}, we use $n=5000$, and the simulation result shows that $M\approx 0.8$ and $K\approx 9$ at $p=2\times 10^4$. Notice that if $n\rightarrow \infty$, then $M\approx 0$, thus $K\approx \infty$, which means that $K$ vanishes in Corollary \ref{coro.wB2_K}.
Nonetheless, we do observe the same shape and trend between our bound and the exact value of $\|\wBP\|_2$, which suggests that our upper bound correctly captures how $\|\wBP\|_2$ changes with key parameters. Further, the exact values of $\|\wBP\|_2$ for $s=1$ and $s=2$ are very close, which is consistent with our conjecture that within the range of $p$ of Theorem \ref{th.main}, the descent speed is not very sensitive to $s$. This phenomenon can also be observed in Fig. \ref{fig.compare_BP_minL2} for larger values of $s$.



==> simulation.tex <==
\section{Numerical Results}
\begin{figure}
    \centering
    \begin{minipage}[t]{0.47\textwidth}
        \centering
\vspace{-0.1in}
        \includegraphics[width=2.8in]{figures/w_I.eps}
        \caption{Bounds of $\|w^I\|_1$ and its exact value, where $\|\etr\|_2=0.01$, $ n=20$.}
        \label{fig.wI}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.47\textwidth}
        \centering
\vspace{-0.1in}
        \includegraphics[width=2.8in]{figures/M.eps}
        \caption{The value of $M$ and its upper bounds (given in Proposition \ref{prop.M}) for the cases of $n=300$ and $n=1200$.}
        \label{fig.M}
    \end{minipage}
\vspace{-0.35in}
\end{figure}



In this section, we provide numerical results that verify our analytic results in earlier sections. We simulate BP in the setting described in Section \ref{sec.system_model}. The first set of numerical results verifies our bounds for $\|w^I\|_1$ and $M$.


In Fig. \ref{fig.wI}, we draw the lower and upper bounds on $\|w^I\|_1$ as $(p-s)$ increases, for the setting of $\|\etr\|_2=0.01$ and $n=20$. The blue curve ``ub, Prop. \ref{prop.bound_WI1}" denotes our theoretical upper bound on $\|w^I\|_1$ (here we use a more detailed form that is tighter than Proposition \ref{prop.new_WI}, which is given in Proposition \ref{prop.bound_WI1} in Appendix \ref{app.proof_of_lemma_12}). 
In the proof of Proposition \ref{prop.new_WI}, we use the idea that $\|w^I\|_1$ is mostly determined by the columns of $\Xtr$ that are closest to the direction of $\etr$. Specifically, among the last $(p-s)$ columns of $\Xtr$, we order them based on the absolute values of their inner-products with $\etr$, and choose $5n$ columns $\mathbf{B}_{(1)},\cdots,\mathbf{B}_{(5n)}$ with the largest values such that $|\mathbf{B}_{(1)}^T\etr|\geq|\mathbf{B}_{(2)}^T\etr|\geq\cdots\geq|\mathbf{B}_{(5n)}^T\etr|$. The upper bounds in Propositions \ref{prop.bound_WI1} and \ref{prop.new_WI} are derived based on the probability distribution of these columns. In contrast, using the \emph{exact} values of these columns, we can construct even tighter bounds on $\|w^I\|_1$. Specifically, in Fig. \ref{fig.wI}, the yellow curve ``ub, use $\mathbf{B}_{(5n)}$" denotes a tighter upper bound on $\|w^I\|_1$ constructed by using the exact value of $\mathbf{B}_{(5n)}$ (see Corollary \ref{coro.bound_by_Aq} in Appendix \ref{app:proof:wI}). The green curve ``ub, use $\mathbf{B}_{(1)}$ to $\mathbf{B}_{(5n)}$" denotes yet another upper bound on $\|w^I\|_1$ constructed by using the exact values of  $\mathbf{B}_{(1)},\cdots, \mathbf{B}_{(5n)}$ (see problem \eqref{prob.temp1} in Appendix \ref{app:proof:wI}). The red curve ``real value" denotes the real value of $\|w^I\|_1$. The purple curve ``lb, use $\mathbf{B}_{(1)}$" denotes the lower bound in Lemma \ref{le.true_lower_bound_WI} of Appendix \ref{app:lower_bounds} using the exact value of $\mathbf{B}_{(1)}$. The first thing that we can verify is that $\|w^I\|_1$ decreases when $(p-s)$ increases. Further, the speed of decrease is relatively slow (notice that the x-axis is in $\log$ scale). In Fig. \ref{fig.wI}, we can see that all curves gets closer when $p$ increases, which implies that our upper bound on $\|w^I\|_1$ is tight. Further, we find that the upper bound using $\mathbf{B}_{(1)}$ to $\mathbf{B}_{(5n)}$ (green curve) almost overlaps with the exact value of $\|w^I\|_1$ (red curve), which verifies our intuition that these columns determine the value of $\|w^I\|_1$.
\begin{figure}
    \centering
    \begin{minipage}[t]{0.47\textwidth}
        \centering
\vspace{-0.1in}
        \includegraphics[width=2.8in]{figures/wB.eps}
        \caption{Exact values and upper bounds of $\|\wBP\|_2$ for cases of $s=1$ and $s=2$, where  $\|\beta\|_2=1$, $\|\etr\|_2=0.01$, $n=3000$.}
        \label{fig.WB}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.47\textwidth}
        \centering
\vspace{-0.1in}
        \includegraphics[width=2.8in]{figures/change_n.eps}
        \caption{Curves of $\|\wBP\|_2$ with different $n$, where $\|\beta\|_2=1$, $\|\etr\|_2=0.01$, $s=1$.}
        \label{fig.change_n}
    \end{minipage}
\vspace{-0.35in}
\end{figure}


In Fig. \ref{fig.M}, we compare the upper bound on $M$ (given in Proposition \ref{prop.M}) with its exact value. We show two cases, $n=300$ (red curves) and $n=1200$ (blue curves). For each case, we can see that the derived upper bound and the exact value of $M$ only differ by a constant factor, which verifies the tightness of our upper bound on $M$ in Proposition \ref{prop.M}.
% When $p=10^4$, those four curves have the value $[1.85, 0.701, 0.496, 0.253]$, from the highest to the lowest, respectively. 
The curve of the exact value of $M$ for $n=1200$ also differs with that for $n=300$ by a constant factor, which is close to $2=\sqrt{1200/300}$. This figure thus validates our conclusion that $M$ is approximately proportional to $1/\sqrt{n}$ for a fixed $p$.


The next set of numerical results directly shows the performance of BP via the model error $\|\wBP\|_2$.
%
In Fig. \ref{fig.WB}, we draw the value of $\|\wBP\|_2$ and its upper bound in Corollary \ref{coro.wB2_K} for cases of $s=1$ and $s=2$. 
All curves are computed using the exact value of $M$ and $\|w^I\|_1$, since we have already shown that our estimates on $M$ and $\|w^I\|_1$ are tight. We see that there is still a relatively large gap between our bound and the real value of $\|\wBP\|$ suggesting room for more refined analysis. 
% One possible reason is that, $n$ is not big enough, thus $K$ in Corollary \ref{coro.wB2_K} introduce a relatively significant constant factor. In Fig. \ref{fig.WB}, we use $n=5000$, and the simulation result shows that $M\approx 0.8$ and $K\approx 9$ at $p=2\times 10^4$. Notice that if $n\rightarrow \infty$, then $M\approx 0$, thus $K\approx \infty$, which means that $K$ vanishes in Corollary \ref{coro.wB2_K}.
Nonetheless, we do observe the same shape and trend between our bound and the exact value of $\|\wBP\|_2$, which suggests that our upper bound correctly captures how $\|\wBP\|_2$ changes with key parameters. Further, the exact values of $\|\wBP\|_2$ for $s=1$ and $s=2$ are very close, which is consistent with our conjecture that within the range of $p$ of Theorem \ref{th.main}, the descent speed is not very sensitive to $s$. This phenomenon can also be observed in Fig. \ref{fig.compare_BP_minL2} for larger values of $s$.


\begin{wrapfigure}{r}{0.47\textwidth}
    \centering
\vspace{-0.1in}
        \includegraphics[width=2.8in]{figures/change_noise.eps}
        \caption{Curves of $\|\wBP\|_2$ with different $\|\etr\|_2$, where $\|\beta\|_2=1$, $s=1$, $n=100$.}
        \label{fig.change_noise}
\vspace{-0.35in}
\end{wrapfigure}

In the rest of this section, we will use Fig.~\ref{fig.change_n}, Fig.~\ref{fig.change_noise}, and Fig.~\ref{fig.compare_BP_minL2} to further verify how  $\|\wBP\|_2$ changes with $n$, $\|\etr\|_2$, and $s$, respectively.
First, we show how $n$ affects $\|\wBP\|_2$. In Fig.~\ref{fig.change_n},
we draw three curves of $\|\wBP\|_2$ for $n=100$, $n=250$, and $n=500$,
respectively. We set $\|\beta\|_2=1,\ \|\etr\|_2=0.01$ and $s=1$. From
Fig. \ref{fig.change_n}, we find that when $p$ is relatively small (when
all three curves are in the decreasing region), $\|\wBP\|_2$ is larger
when $n$ increases. This is consistent with the trend predicted by our
upper bound in Theorem \ref{th.main}. On the other hand, as $p$
increases, the lowest points of all three curves for different $n$ are
very close. This observation verifies our conclusion in Corollary
\ref{coro.only_s} that the descent floor is independent of~$n$. 

%Next, we
%will show how $s$ affects $\|\wBP\|_2$.  In Fig. \ref{fig.change_s}, we
%draw three curves of $\|\wBP\|_2$ for $s=1$, $s=4$, and $s=16$,
%respectively. We set $\|\beta\|_2=1,\ \|\etr\|_2=0.01$ and $n=100$. The
%lowest values (i.e., the descent floors) of those three curves are
%$[0.0050, 0.0084, 0.0160]$ for $s=1$, $s=4$, $s=16$ respectively. Thus,
%we find that the descent floor are nearly proportional to $\sqrt{s}$.

% \begin{figure}
%     \centering
%     \begin{minipage}[t]{0.47\textwidth}
%         \centering
% \vspace{-0.1in}
%         \includegraphics[width=2.8in]{figures/change_s.eps}
%         \caption{Curves of $\|\wBP\|_2$ with different $s$, where $\|\beta\|_2=1$, $\|\etr\|_2=0.01$, $n=100$.}
%         \label{fig.change_s}
%     \end{minipage}\hfill
%     \begin{minipage}[t]{0.47\textwidth}
%         \centering
% \vspace{-0.1in}
%         \includegraphics[width=2.8in]{figures/change_noise.eps}
%         \caption{Curves of $\|\wBP\|_2$ with different $\|\etr\|_2$, where $\|\beta\|_2=1$, $s=1$, $n=100$.}
%         \label{fig.change_noise}
%     \end{minipage}
% \vspace{-0.35in}
% \end{figure}



\begin{figure}
    \centering
%\vspace{-0.1in}
    \includegraphics[width=4.5in]{figures/compare_BP_minL2_new.eps}
\vspace{-0.20in}
        \caption{Compare BP with min $\ell_2$-norm, where $\|\etr\|_2=0.01$, $ n=500$.}
        \label{fig.compare_BP_minL2}
\vspace{-0.1in}
\end{figure}

Next, we show how $\|\etr\|_2$ affects $\|\wBP\|_2$. In Fig.
\ref{fig.change_noise}, we draw three curves of $\|\wBP\|_2$ with
different $\|\etr\|_2$. The lowest values of those three curves are
$[0.005, 0.023, 0.081]$ for $\|\etr\|_2=0.01$, $\|\etr\|_2=0.04$, and
$\|\etr\|_2=0.16$, respectively. We find that the lowest values are
nearly proportional to $\|\etr\|_2$. 
% Further, as $p$ increases,
% eventually the model error will increase, which is more evident when $s$
% is large ($s=16$). We will report the dependency on $s$ in
% Fig.~\ref{fig.compare_BP_minL2} below. 

% \begin{wrapfigure}{r}{0.75\textwidth}
%     \centering
% \vspace{-0.1in}
%     \includegraphics[width=4.0in]{figures/compare_BP_minL2_new.eps}
%         \caption{Compare BP with min $\ell_2$-norm, where $\|\beta\|_2=1$, $\|\etr\|_2=0.01$, $ n=500$.}
%         \label{fig.compare_BP_minL2}
% \vspace{-0.35in}
% \end{wrapfigure}
In Fig. \ref{fig.compare_BP_minL2}, we compare BP with the
overfitting solution that minimizes the $\ell_2$-norm. We consider both
the sparse ($s=1$) and not sparse ($s=100$) situations, as well as two
different values of $\|\beta\|_2=1$ and $\|\beta\|_2=0.1$. 
%All four curves
We can observe the descent floors of both algorithms. However,  
comparing the curves with the same $s=100$, we can see that the descent
floors (the lowest points of the curves) of min $\ell_2$-norm solutions vary significantly with
$\|\beta\|_2$, while those of BP are insensitive to $\|\beta\|_2$.
Further, comparing the curves with the same $\|\beta\|_2=1$, we can see
that 
%report the model error $\|w\|_2$ as $p$ increase. Note that all four
%curves decreases sharply when $p$ is a little larger than $n$,
%suggesting the ``double decent" phenomenon.  However, consistent with
%our discussions after Corollary \ref{coro.only_s}, 
the descent floors of
BP are significantly lower and wider than that of min $\ell_2$-norm
overfitting solutions (note that $\|\etr\|_2=0.01\ll \|\beta\|_2=1$).
%Indeed, in the case of $s=1$, the model error of BP keeps decreasing
%within the whole range of $p$ in this figure. 
This result thus
demonstrates the performance advantage of using BP in similar regimes.
% However, we also find significant differences between BP (i.e., minimizing $\ell_1$-norm) and the min $\ell_2$-norm solution. For the min $\ell_2$-norm solution, regardless of $s=1$ or $s=100$, the model error approaches $\|\beta\|_2=1$ (i.e., the ``null risk") when $p$ is large. In the case of $s=100$, although the model error of BP also eventually increases with $p$ (after the decrease at the beginning), BP has a much larger region of descent than that of the min $\ell_2$-norm solution. In the case of $s=1$, the model error of BP keeps decreasing withing the range of $p$ in this figure. In both cases, BP has a lower descent floor than the min $\ell_2$-norm solution.
% In summary, we conclude that, when the number of parameters and the dimension of the data are both much larger than the number of samples, BP performs significantly better than min $\ell_2$-norm solutions in achieving lower model error while overfitting the data.
%
Finally, for the two curves for BP with $\|\beta\|_2=1$ but
different sparsity levels $s$, 
%Next, we
%will show how $s$ affects $\|\wBP\|_2$.  In Fig. \ref{fig.change_s}, we
%draw three curves of $\|\wBP\|_2$ for $s=1$, $s=4$, and $s=16$,
%respectively. We set $\|\beta\|_2=1,\ \|\etr\|_2=0.01$ and $n=100$. The
we can see that the descent floors (the lowest points) 
%%of those three curves are
%$[0.0050, 0.0084, 0.0160]$ for $s=1$, $s=4$, $s=16$ respectively. Thus,
%we find that the descent floor 
are nearly proportional to $\sqrt{s}$, which confirms the result in
Corollary~\ref{coro.only_s}.



==> simulation_arXiv.tex <==
\section{Numerical Results}

\linx{How much of this section will be kept?}


In this section, we provide numerical results that verify our analytic results in earlier sections. We simulate BP in the setting described in Section \ref{sec.system_model}. The first set of numerical results verifies our bounds for $\|w^I\|_1$ and $M$.


\begin{comment}
\begin{figure}
    \centering
    \begin{minipage}[t]{0.47\textwidth}
        \centering
        \includegraphics[width=2.8in]{figures/change_noise.eps}
        \caption{Curves of $\|\wBP\|_2$ with different $\|\etr\|_2$, where $\|\beta\|_2=1$, $s=1$, $n=100$.}
        \label{fig.change_noise}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.47\textwidth}
        \centering
        \includegraphics[width=2.8in]{figures/change_n.eps}
        \caption{Curves of $\|\wBP\|_2$ with different $n$, where $\|\beta\|_2=1$, $\|\etr\|_2=0.01$, $s=1$.}
        \label{fig.change_n}
    \end{minipage}
\end{figure}
\end{comment}

% \begin{wrapfigure}{r}{0.47\textwidth}
%     \centering
%         \includegraphics[width=2.8in]{figures/change_noise.eps}
%         \caption{Curves of $\|\wBP\|_2$ with different $\|\etr\|_2$, where $\|\beta\|_2=1$, $s=1$, $n=100$.}
%         \label{fig.change_noise}
% \end{wrapfigure}



The next set of numerical results directly shows the performance of BP
via the model error $\|\wBP\|_2$.
%

In the rest of this section, we will use Fig.~\ref{fig.change_n}, Fig.~\ref{fig.change_noise}, and Fig.~\ref{fig.compare_BP_minL2} to further verify how  $\|\wBP\|_2$ changes with $n$, $\|\etr\|_2$, and $s$, respectively.
First, we show how $n$ affects $\|\wBP\|_2$. In Fig.~\ref{fig.change_n},
we draw three curves of $\|\wBP\|_2$ for $n=100$, $n=250$, and $n=500$,
respectively. We set $\|\beta\|_2=1,\ \|\etr\|_2=0.01$ and $s=1$. From
Fig. \ref{fig.change_n}, we find that when $p$ is relatively small (when
all three curves are in the decreasing region), $\|\wBP\|_2$ is larger
when $n$ increases. This is consistent with the trend predicted by our
upper bound in Theorem \ref{th.main}. On the other hand, as $p$
increases, the lowest points of all three curves for different $n$ are
very close. This observation verifies our conclusion in Corollary
\ref{coro.only_s} that the descent floor is independent of~$n$. 

%Next, we
%will show how $s$ affects $\|\wBP\|_2$.  In Fig. \ref{fig.change_s}, we
%draw three curves of $\|\wBP\|_2$ for $s=1$, $s=4$, and $s=16$,
%respectively. We set $\|\beta\|_2=1,\ \|\etr\|_2=0.01$ and $n=100$. The
%lowest values (i.e., the descent floors) of those three curves are
%$[0.0050, 0.0084, 0.0160]$ for $s=1$, $s=4$, $s=16$ respectively. Thus,
%we find that the descent floor are nearly proportional to $\sqrt{s}$.

% \begin{figure}
%     \centering
%     \begin{minipage}[t]{0.47\textwidth}
%         \centering
% \vspace{-0.1in}
%         \includegraphics[width=2.8in]{figures/change_s.eps}
%         \caption{Curves of $\|\wBP\|_2$ with different $s$, where $\|\beta\|_2=1$, $\|\etr\|_2=0.01$, $n=100$.}
%         \label{fig.change_s}
%     \end{minipage}\hfill
%     \begin{minipage}[t]{0.47\textwidth}
%         \centering
% \vspace{-0.1in}
%         \includegraphics[width=2.8in]{figures/change_noise.eps}
%         \caption{Curves of $\|\wBP\|_2$ with different $\|\etr\|_2$, where $\|\beta\|_2=1$, $s=1$, $n=100$.}
%         \label{fig.change_noise}
%     \end{minipage}
% \vspace{-0.35in}
% \end{figure}





Next, we show how $\|\etr\|_2$ affects $\|\wBP\|_2$. In Fig.
\ref{fig.change_noise}, we draw three curves of $\|\wBP\|_2$ with
different $\|\etr\|_2$. The lowest values of those three curves are
$[0.005, 0.023, 0.081]$ for $\|\etr\|_2=0.01$, $\|\etr\|_2=0.04$, and
$\|\etr\|_2=0.16$, respectively. We find that the lowest values are
nearly proportional to $\|\etr\|_2$. 
% Further, as $p$ increases,
% eventually the model error will increase, which is more evident when $s$
% is large ($s=16$). We will report the dependency on $s$ in
% Fig.~\ref{fig.compare_BP_minL2} below. 

% \begin{wrapfigure}{r}{0.75\textwidth}
%     \centering
% \vspace{-0.1in}
%     \includegraphics[width=4.0in]{figures/compare_BP_minL2_new.eps}
%         \caption{Compare BP with min $\ell_2$-norm, where $\|\beta\|_2=1$, $\|\etr\|_2=0.01$, $ n=500$.}
%         \label{fig.compare_BP_minL2}
% \vspace{-0.35in}
% \end{wrapfigure}
In Fig. \ref{fig.compare_BP_minL2}, we compare BP with the
overfitting solution that minimizes the $\ell_2$-norm. We consider both
the sparse ($s=1$) and not sparse ($s=100$) situations, as well as two
different values of $\|\beta\|_2=1$ and $\|\beta\|_2=0.1$. 
%All four curves
We can observe the descent floors of both algorithms. However,  
comparing the curves with the same $s=100$, we can see that the descent
floors (the lowest points of the curves) of min $\ell_2$-norm solutions vary significantly with
$\|\beta\|_2$, while those of BP are insensitive to $\|\beta\|_2$.
Further, comparing the curves with the same $\|\beta\|_2=1$, we can see
that 
%report the model error $\|w\|_2$ as $p$ increase. Note that all four
%curves decreases sharply when $p$ is a little larger than $n$,
%suggesting the ``double decent" phenomenon.  However, consistent with
%our discussions after Corollary \ref{coro.only_s}, 
the descent floors of
BP are significantly lower and wider than that of min $\ell_2$-norm
overfitting solutions (note that $\|\etr\|_2=0.01\ll \|\beta\|_2=1$).
%Indeed, in the case of $s=1$, the model error of BP keeps decreasing
%within the whole range of $p$ in this figure. 
This result thus
demonstrates the performance advantage of using BP in similar regimes.
% However, we also find significant differences between BP (i.e., minimizing $\ell_1$-norm) and the min $\ell_2$-norm solution. For the min $\ell_2$-norm solution, regardless of $s=1$ or $s=100$, the model error approaches $\|\beta\|_2=1$ (i.e., the ``null risk") when $p$ is large. In the case of $s=100$, although the model error of BP also eventually increases with $p$ (after the decrease at the beginning), BP has a much larger region of descent than that of the min $\ell_2$-norm solution. In the case of $s=1$, the model error of BP keeps decreasing withing the range of $p$ in this figure. In both cases, BP has a lower descent floor than the min $\ell_2$-norm solution.
% In summary, we conclude that, when the number of parameters and the dimension of the data are both much larger than the number of samples, BP performs significantly better than min $\ell_2$-norm solutions in achieving lower model error while overfitting the data.
%
Finally, for the two curves for BP with $\|\beta\|_2=1$ but
different sparsity levels $s$, 
%Next, we
%will show how $s$ affects $\|\wBP\|_2$.  In Fig. \ref{fig.change_s}, we
%draw three curves of $\|\wBP\|_2$ for $s=1$, $s=4$, and $s=16$,
%respectively. We set $\|\beta\|_2=1,\ \|\etr\|_2=0.01$ and $n=100$. The
we can see that the descent floors (the lowest points) 
%%of those three curves are
%$[0.0050, 0.0084, 0.0160]$ for $s=1$, $s=4$, $s=16$ respectively. Thus,
%we find that the descent floor 
are nearly proportional to $\sqrt{s}$, which confirms the result in
Corollary~\ref{coro.only_s}.


